An off-the-grid approach to multi-compartment magnetic resonance fingerprinting

We propose a novel numerical approach to separate multiple tissue compartments in image voxels and to estimate quantitatively their nuclear magnetic resonance (NMR) properties and mixture fractions, given magnetic resonance fingerprinting (MRF) measurements. The number of tissues, their types or quantitative properties are not a-priori known, but the image is assumed to be composed of sparse compartments with linearly mixed Bloch magnetisation responses within voxels. Fine-grid discretisation of the multi-dimensional NMR properties creates large and highly coherent MRF dictionaries that can challenge scalability and precision of the numerical methods for (discrete) sparse approximation. To overcome these issues, we propose an off-the-grid approach equipped with an extended notion of the sparse group lasso regularisation for sparse approximation using continuous (non-discretised) Bloch response models. Further, the nonlinear and non-analytical Bloch responses are approximated by a neural network, enabling efficient back-propagation of the gradients through the proposed algorithm. Tested on simulated and in-vivo healthy brain MRF data, we demonstrate effectiveness of the proposed scheme compared to the baseline multicompartment MRF methods.

==> sections/expe.tex <==
\section{Experiments}
Computations were conducted using MATLAB on an Intel Xeon gold CPU core and 32 GB RAM. %and a NVIDIA 2080Ti GPU. 
In the spirit of reproducible research, the source codes of the proposed algorithms are available at \todo{...}. 

All experiments (simulated and \emph{in-vivo}) adopted a joint T1/T2-encoding MRF excitation sequence similar to the Fast Imaging Steady State Precession (FISP) protocol~\cite{FISP} using the same flip angle schedule, fixed TR/TE = 10/1.9 ms, and inversion time 18 ms. This sequence had the length of $T=1000$ timepoints (repetitions). 

\subsection{Tested algorithms}
%For FISP MRF sequence with constant TE per-voxel signal evolution has a constant complex-valued phase~\nref[doneva]. This  phase can be estimated from the first principal components of the dimension-reduced TSMI and removed from the image~\cite{AIRMRF, coverblip_iop, MRFLRTV}. 
We compared \MCMRF (Algorithm~\ref{alg:FW}) to the MC-MRF baselines SPIJN~\cite{SPIJN}, BayesianMRF~\cite{BayesianPVMRF} and PVMRF~\cite{PVMRF}. All algorithms used subspace dimensionality reduction $\tau=10$~\cite{SVDMRF,MRFLRTV}. Reconstructed TSMIs were phase-corrected and mapped to real-valued images before applying mixture separation. 
%For in-vivo scans we used coil sensitivities computed from undersampled data using an adaptive coil combination scheme~\cite{adaptivesense}. 
Baselines work with fine-gridded MRF dictionary dictionaries. 
In Section~\ref{sec:vivo} we also compared a discretised variant of
our algorithm, named SG-Lasso~\cite{SPGLasso}, 
%, that solves the sparse group lasso problem~\cite{SPGLasso}
using the same  MRF dictionary as the baselines. Methods' parameters were grid searched and chosen based on scoring low model errors to~\eqref{eq:model4}, visual separability of the mixture maps, and consistency of the estimated T1/T2 values with respect to the ground-truth (simulations) or literature values (in-vivo).
%Unless otherwise specified the used parameters were as follows: 
The regularisation parameters of BayesianMRF and SPIJN were $\mu_{\text{B}}=\{0.001,1\}$ and $\la_{\text{SPIJN}}=\{0.03,0.7\}$ for dirichlet phantoms %(section~\ref{sec:diri_expe}) 
and in-vivo experiments, respectively. BayesianMRF used shape parameters $\alpha_{\text{B}}=1.75, \beta_{\text{B}}=0.1$. PVMRF used parameter $k_{\text{PVMRF}}=11$ for the k-means. To stabilise PVMRF, 
 %and BayesianMRF algorithms, the involved  
 k-means steps were repeated 10 times (randomly initialised) and result scoring lowest model error~\eqref{eq:model4} was selected. \MCMRF used parameters $\alpha=10^{-6},\beta=0.9$ for dirichlet phantoms experiment and $\alpha=0.8,\beta=10^{-3}$ for the simulated and in-vivo brain experiments. 


\subsection{Embedding Bloch responses by neural network} 
\label{sec:expe_neural}

%We also examined effects of shorter acquisitions through truncating the length of this sequence.
A neural network was trained to approximate Bloch responses.  
%(different network per sequence length). 
For training and evaluation 95'143 Bloch responses were simulated using the Extended Phase Graph (EPG) formalism~\cite{EPGWeigel} over a (T1,T2) $\in [10, 6000]$ ms $\times[4,4000]$ ms grid discretised by logarithmically spaced values of T1 and T2 (400 points each) with T1 $>$ T2 constraint. PCA was applied to compress Bloch responses' temporal dimensions to a $\tau=10$ dimensional subspace~\cite{SVDMRF}.  
Data was randomly splitted in $80-10-10$ precent ratios for training, validation and testing sets, correspondingly. %The size and topology of the networks are application dependant. 
For our application we followed~\cite{MRFLRTV} and used a small size (convolutional) network with $1\times1$ filters for pixel-wise processing: 2-channel inputs for T1 and T2 values, 10-channel (linear) outputs for compressed Bloch responses, and one hidden layer of 500 channels with nonlinear ReLU activations.  
%Neurons are fully connected and networks process individual image voxels in one full Batch size of the foreground image pixels during testing.  
%Neurons are fully connected and process individual image voxels received in batches. 
For training we minimised the MSE loss between the EPG-generated and network-predicted (dimension-reduced) Bloch responses using ADAM optimiser ran for 100 epochs with initial learning rate $0.005$, learning rate/gradient decay factors $0.95/0.95$, and minibatch size $100$. Training and validation curves are shown in supplementary materials, Figure~\ref{fig:trainingcurve}. Training, validation and testing normalised RMSEs for approximating Bloch responses were $\{8.9397, 8.9742, 8.9561\}\times10^{-3}$, correspondingly. 
%\todo{Data was randomly spitted to 80\%-20\% ratios for training and validation sets correspondingly, and 10'000 randomly sampled test data points out of these sets were used for testing set.}
%\todo{The accuracy of the network predictions are reported in Table\nref for 10'000 randomly sampled test data points (out-of-the training set), indicating less than XX\% difference with the EPG generated Bloch responses.}  

%%=====TABLE==============================
%\begin{table}[h!]
%	%\vspace{0cm}
%	\centering
%	\scalebox{1}{
%		\begin{tabular}{c|c|c|c|c}
%			\toprule[0.2em]
%			NRMSE $\backslash$ $T$& $1000$ &$750$&$500$& $250$  \\	
%			\midrule[0.05em]	
%			\midrule[0.05em]		
%			Training  &8.9397e-03 & 1.2615e-02 & 3.2772e-02 & 6.0961e-02\\	
%			\midrule[0.1em]	
%			Testing  & 8.9561e-03 & 1.2582e-02 & 3.2252e-02 & 6.1495e-02\\			
%			\bottomrule[0.2em]
%		\end{tabular}		}
%		\caption{Training and testing Normalised RMSE for approximating Bloch responses of lengths $T$ using neural networks.  \todo{the numbers should not increase}}
%		\label{tab:DNN}
%	\end{table}
%%=======================================

Only \MCMRF used neural network approximations. 
For the initialising grid-search in step 2, a fixed 64-atom dictionary was simulated over 10 logarithmically-spaced points per T1 and T2, respecting T1$>$T2.
Tested baselines used the actual EPG dictionary comprising 8'540 
%(size typically used in previous works) subspace-compressed 
 fingerprints  simulated on a logarithmically spaces grid; 
 % (T1,T2) $\in [10, 6000]$ ms $\times[4,4000]$ ms; 
 120 values for per T1 and T2. %, respecting T1$>$T2. 

%=======diri_algos
\begin{figure}[t]
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=\linewidth]{../figs_gen/synth/figs_expe2/expe2_diri_algo.pdf}
\caption{{The T1 (top) and T2 (bottom) MAPE errors of the MC-MRF algorithms for estimating dirichlet phantoms' compartments with different mixture parameters $a$. Plots are cropped to 100\% MAPE and colour-coded for different algorithms. 10 independent phantoms were simulated/demixed per $a$ value.}\label{fig:synth_diri} }
\end{minipage}
\end{figure}

%=======noise grid
\begin{figure}[t]
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=\linewidth]{../figs_gen/synth/figs_expe5/expe5_noise_grid.pdf}
\caption{{The T1 (top) and T2 (bottom) MAPE errors for estimating the numerical box phantom's compartments (dirichlet mixture $a=0.5$) using \MCMRF algorithm with different initialising grid sizes and different SNR (dB) levels. 10 independent phantoms were simulated/demixed per SNR value.}\label{fig:synth_gidnoise} }
\end{minipage}
\end{figure}

 


%\subsection{Simulated data}
\subsection{Numerical dirichlet phantoms experiment}
\label{sec:diri_expe}

A number of phantoms were simulated according to the mixture model~\eqref{eq:model2} for creating TSMIs 
of $20\times20$ pixels spatial resolutions and $T=1000$ length timeframes. In these phantoms three compartments were used  with relaxation properties T1/T2 $=\{784/77, 1216/96, 4083/1394\}$ ms. 
%, mimicking the 1.5 Tesla literature values\nref for white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF). 
Per-pixel mixture weights were drawn independently at random from dirichlet distributions parametrised by various values of $a>0$. This parameter governs the mixture levels such that  large $a$ values result in highly mixed pixels that receive similar contributions from all compartments and hence are more difficult for demixing~\cite{bioucas_sisal}. On the other hand small $a$ lead to sparse mixture maps i.e. pixels receive contributions from fewer compartments, making demixing task easier. 

We created a dataset of such phantoms from different mixture distributions with values $a\in\{0.1,0.5,1,2,4\}$ and for each distribution we simulated 10 phantoms independently at random (see exemplar mixtures in Fig~\ref{fig:diri_maps}, 
supplementary materials). We used this dataset to compare the performances of MC-MRF baselines with the \MCMRF algorithm. Evaluation metrics were the Mean Absolute Percentage Errors (MAPE) of T1 and T2 values of the recovered compartments with respect to the ground truth values. Results are reported in box plots in Figure~\ref{fig:synth_diri}. The \MCMRF outperforms tested baselines with accurate T1/T2 estimations i.e. less than \%5 average errors, for all tested mixture distributions. For $a=0.1$ where mixtures are extremely sparse the PVMRF and SPIJN methods perform comparably well. However \MCMRF shows robustness for separating more dense mixtures i.e. lager $a$ values, where the gap between baselines and \MCMRF both in terms of the median and variance of the MAPE errors increases.

In another experiment we created a dataset of phantoms by setting the parameter $a=0.5$ and corrupt the TSMIs by additive white gaussian noises of various SNRs $\in\{10, 20, 30, 40, 60\}$ dB. 
We simulated 10 noisy phantoms per SNR value. 
%We used this data to access the stability of \MCMRF with respect to noise and the size of the grid search step used in the Frank-Wolfe Algorithm\nref. 
We used this dataset to measure the sensitivity of \MCMRF to noise and also size of the grid-search used in Algorithm~\ref{alg:FW} (step 2). For this we increased the storage requirement of \MCMRF using grid-sizes  \{64, 991, 2237\} corresponding to sampling  \{10,  40, 60\} logarithmically-spaced points per T1 and per T2, where T1$>$T2. 
 The estimated T1 and T2 MAPEs are reported in Figure~\ref{fig:synth_gidnoise}. For SNRs $\geq20$ dB the average errors are less than \%5. Errors then increase to \%10-\%15 in the lowest tested SNR regime 10 dB. Further, it can be observed that \MCMRF's overall performance per SNR regime has small variations with respect to the tested grid-sizes (less than \%3 difference on average MAPEs) which could motivate the adoption of small grid-sizes to overcome the memory inefficiency (challenge of dimensionality) of the dictionary-based MC-MRF approaches. In all other experiments throughout this paper, \MCMRF used the smallest grid-size 64 that is 2 orders of magnitude smaller and more memory-efficient than the grid-size (i.e. 8'540 fingerprints) of the MRF dictionaries used by the baselines.


%=====brainweb GTmaps=====
\begin{figure}[t]
	\centering
	\scalebox{.95}{
	\begin{minipage}{\linewidth}
		\centering		
\includegraphics[width=.32\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/GT1c.pdf}
\includegraphics[width=.32\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/GT2c.pdf}
\includegraphics[width=.32\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/GT3c.pdf}
\caption{{Ground truth mixture maps for the Brainweb phantom. 
}\label{fig:brainweb_GTmaps} }
\end{minipage}}
\end{figure}

%===================

%================
\begin{figure}[t]
	\centering
	\scalebox{1}{
	\begin{minipage}{\linewidth}
		\centering		
\includegraphics[width=\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_MAPE_boxchart.pdf}\\
\includegraphics[width=\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_PSNR_boxchart.pdf}\\
\includegraphics[width=\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_SSIM_boxchart.pdf}
\caption{{The T1/T2 MAPE errors, mixture maps' PSNR and SSIM for estimating the WM, GM, CSF compartments of the simulated brain phantom, using \MCMRF. For various sequence lengths $T$, the TSMIs were either un-compressed (Full) or compressed sampled and reconstructed with the LRTV and SVD-MRF schemes before mixture separation.}
%with different grid sizes. Sub-sampled k-space measurements with different SNRs were fed to \MCMRF\ using different grid sizes. Errors are averaged over 10 independent trials for each SNR.}
\label{fig:barinweb_boxchart} }
\end{minipage}}
\end{figure}
%=====================

%=======	

\begin{table*}[t!]
	%\vspace{0cm}
	\centering
	\fontsize{9}{9}\selectfont
	\scalebox{.9}{
		\begin{tabular}{ccc|ccc|ccc}
			\toprule[0.2em]
			\multicolumn{3}{c}{WM} & \multicolumn{3}{c}{GM} & \multicolumn{3}{c}{CSF}\\
			\midrule[0.1em]
%			\multicolumn{1}{c}{} &\multicolumn{2}{c}{MAPE (\%)} & \multicolumn{2}{c}{MAE (ms)} & \multicolumn{2}{c}{SNR (dB)} & \multicolumn{3}{c}{SSIM}  &  \multicolumn{2}{c}{MAPE (\%)} & \multicolumn{2}{c}{MAE (ms)} & \multicolumn{2}{c}{SNR (dB)} &\multicolumn{3}{c}{SSIM}  \\
%			\midrule[0.1em]
			{T1/T2 MAPE} &{PSNR} & {SSIM} &   {T1/T2 MAPE} &{PSNR} & {SSIM} & {T1/T2 MAPE} &{PSNR} & {SSIM}  \\
			\midrule[0.05em]
			\midrule[0.05em]
			 $5.33/2.23$ & $24.17$ & $0.855$ & $0.30/1.59$ & $23.29$& $0.934$ & $1.97/2.99$ & $36.62$ & $0.957$\\
			%\midrule[0.05em]
			
			\midrule[0.1em]
			
			$5.02/3.04$ & $21.26$ & $0.805$ & $0.60/0.45$ & $19.62$  & $0.889$ & $0.22/21.34$ & $32.00$ & $0.921$ \\
			%\midrule[0.05em]
						
		\bottomrule[0.2em]
		\end{tabular}}
		\caption{ The T1/T2 MAPE (\%) errors and the mixture maps' SSIM and PNSR (dB) using \MCMRF\ and PVMRF methods (both using LRTV reconstruction) for estimating WM, GM, CSF compartments in simulated brain, for different acquisition lengths $T$ and non-exactly sparse (Gaussian-distributed) compartments $r$. Values are averaged over 10 Monte-Carlo runs of the experiments.\todo{add std, besides MAPE ass actual t1/t2 values, add TSMI fidelity}} \vspace{.3cm}\label{tab:expe_simul}
		\end{table*}
	
%%=================

\begin{figure*}[t!]
	\centering
	\scalebox{.95}{
	\begin{minipage}{\linewidth}
		\centering	
		WM \hspace{1.8cm}$\Delta$ WM	\hspace{1.9cm} GM \hspace{2cm}$\Delta$ GM \hspace{1.9cm} CSF\hspace{1.9cm}$\Delta$ CSF\vspace{.1cm}\\
\begin{turn}{90} \quad\qquad Full \end{turn}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1351c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1351.pdf}\hspace{.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1352c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1352.pdf}\hspace{.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1353c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1353.pdf}
\\
\begin{turn}{90} \quad\qquad LRTV \end{turn}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1151c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1151.pdf}\hspace{.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1152c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1152.pdf}\hspace{.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1153c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1153.pdf}
\\
\begin{turn}{90} \qquad SVD-MRF \end{turn}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1251c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1251.pdf}\hspace{.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1252c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1252.pdf}\hspace{.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_1253c.pdf}\hspace{-.1cm}
\includegraphics[width=.15\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/expe3_cut_im_diff_1253.pdf}
\\
\hspace{.2cm}
\includegraphics[width=.13\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/colorbarMaps_c.pdf}\hspace{.3cm}
\includegraphics[width=.13\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/colorbardiffMaps.pdf}\hspace{.3cm}
\includegraphics[width=.13\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/colorbarMaps_c.pdf}\hspace{.3cm}
\includegraphics[width=.13\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/colorbardiffMaps.pdf}\hspace{.3cm}
\includegraphics[width=.13\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/colorbarMaps_c.pdf}\hspace{.3cm}
\includegraphics[width=.13\linewidth]{../figs_gen/brainweb/figs_expe3_cut/mixmaps_new/colorbardiffMaps.pdf}
\end{minipage}}
\caption{{The estimated T1/T2 values, mixture maps and their differences ($\Delta$) with the ground truth for the WM, GM and CSF compartments of the simulated brain phantom using \MCMRF for lengths $T=1000$. TSMIs were either un-compressed (Full) or subsampled using compressed sensing and reconstructed with the LRTV and SVD-MRF schemes before mixture separation. 
}\label{fig:brainweb_SGBlasso_main} }
\end{figure*}

\subsection{Numerical Brain phantom experiment}
\label{sec:brainweb}
This experiment used the Brainweb's anatomical model of healthy brain~\cite{Brainweb-collins, webbrain}. This data includes fuzzy segmentations of the white matter (WM), gray matter (GM) and cerebrospinal fluid (CSF) and provides precise control on the ground truth mixture maps (Figure~\ref{fig:brainweb_GTmaps}). The assigned relaxation properties for these tissues were T1/T2 $=\{784/77, 1216/96, 4083/1394\}$ ms. %, mimicking the 1.5 Tesla literature values\nref for WM, GM and CSF. 
Given these mixture maps and compartments' T1/T2 information the TSMIs were constructed according to the model~\eqref{eq:model2}. % and using EPG Bloch response simulations.  

We used this data to study \MCMRF's performance for the case where TSMIs were un-compressed (fully sampled) and compare it to the case where acquisitions were accelerated through k-space subsampling (i.e. compressed sensing). In the latter case, TSMIs were subsampled using the same k-space readouts used for acquiring in-vivo MRF data (a single channel coil-combined scenario has been simulated). 10 independent realisations of gaussian noise (40 dB SNR) were added to the measurements in each case to form our dataset. Where compressed sensing applied, we adopted the reconstruction schemes LRTV and SVD-MRF to estimate TSMIs before the demixing step and compared their performances. We also studied stability of the methods for shorter acquisitions through truncated excitation sequences for $T=500$ and $250$, besides the original length $T=1000$.


Results are reported in Figure~\ref{fig:barinweb_boxchart} and 
the metrics used for evaluation were the joint T1/T2 MAPE, the mixture map reconstruction PNSR and the mixture map Structural Similarity Index Metric (SSIM), measured per WM, GM and CSF compartments. Figure~\ref{fig:brainweb_SGBlasso_main} also illustrates an example of the reconstructed mixture maps (weights) and their differences to the ground truth, for un-compressed and compressed acquisitions with LRTV and SVD-MRF reconstructions where $T=1000$. Similar illustrations for $T=$ 500 and 200 are included in the supplementary materials Figure~\ref{fig:brainweb_SGBlasso}. 


As can be seen in Figure~\ref{fig:barinweb_boxchart}, for long sequence length $T=1000$ the estimated T1/T2 values are accurate with less than \%5 average MAPEs for all compartments, using full and compressed sampled data. Estimated mixture maps produce larger errors using subsampled data, but this error is smaller using LRTV reconstruction as compared to SVD-MRF which produces strong subsampling (aliasing) artefacts (see Figure~\ref{fig:brainweb_SGBlasso_main} and Figure~\ref{fig:brainweb_SGBlasso}).  For shorter sequences $T$, the SVD-MRF applied to subsampled data shows great instability i.e. higher T1/T2 errors with larger variations and also significant drops in the mixture maps' PSNR and SSIM (e.g. more than 25 dB and 40\% respectively, for $T=250$) compared to the uncompressed phantom. 
However applying LRTV reconstruction prior to \MCMRF creates stability and manages to report closer performance to the un-compressed data over all tested metrics. Here the largest performance loss is due to the CSF's T1/T2 values (not the mixture maps) that are challenging to accurately estimate  in compressed data with short sequence lengths $T$. Otherwise, the WM and GM's T1/T2 average MAPEs remain small (about \%5) for $T=500$ and $250$-lengths compressed data. Further  the mixture maps' are aliased-free,  their SSIMs are all above 80\%, and their PNSRs are larger than 20 dB for WM and GM, and larger than 30 dB for CSF (see also Figures~\ref{fig:brainweb_SGBlasso_main}~and~\ref{fig:brainweb_SGBlasso} for qualitative comparisons).  
%The WM and GM's T1/T2 average MAPEs are also small (about \%5) for $T=500, 250$ and the largest performance loss here is due to the CSF's T1/T2 values (not the mixture maps) that are challenging to estimate accurately in compressed data with short sequence lengths $T$. 

\todo{discuss:This highlighting impoetasntce of adopting good recon prior to \MCMRF}




%\newpage
%
%MC-MRF acquisitions were simulated using Brainweb's anatomical model of healthy brain~\cite{webbrain}. Fuzzy segmentations of the white matter (WM), gray matter (GM) and cerebrospinal fluid (CSF) provided precise control on the ground-truth (GT) mixture maps  (Figure~\ref{fig:brainweb_GTmaps}). The assigned relaxation properties for these tissues were mimicking 1.5T literature values\nref. Per tissue T1/T2 values were distributed at random following i.i.d. Gaussian distributions with the mean $\mu_{\text{WM}}=784/77$ ms and scaled standard deviations $r\sigma_{\text{WM}}=r100/r12$ ms for WM, $\mu_{\text{GM}}=1216/96$ ms and $r\sigma_{\text{GM}}=r200/r12$ ms for GM, and $\mu_{\text{CSF}}=4083/1394$ ms and $r\sigma_{\text{CSF}}=r600/r400$ for CSF. Gaussians' variances where controlled by scale factors $r\in\{0,0.5,1,2\}$. Through varying $r$ we study sensitivity of the algorithms when relaxing the exact sparsity assumption (i.e. $r=0$) on the compartments. 
%Given the mixture maps and multi-compartment T1/T2 distributions, TSMIs were constructed according to the mixture model~\eqref{eq:model3} and using EPG Bloch response simulations. TSMIs were then sub-sampled using the same k-space readouts used for acquiring in-vivo data (a single channel coil-combined scenario has been simulated). K-space measurements where corrupted by SNR$=40$ dB i.i.d. Gaussian noise. 
%\todo{no need for shorter, they're inconsistent}We also studied stability of the methods for shorter acquisitions through truncated sequences as mentioned above for fixed SNR$=40$ dB and $r=0$. For each studied $r$ factor or sequence length, the entire experiment process was repeated 10 times in a Monte Carlo fashion. %for independent 
%Finally we used this data (fixed $r=0$, $T=1000$) to measure sensitivity of the proposed algorithm to the grid-size used for \todo{initialising Blasso's search step} for various SNRs of $20,30,40$ and $60$ dB. 
%For this we gradually increased the storage requirement of \MCMRF to finally match that of the dictionary-based MC-MRF baselines using grid-sizes 
%%\{64, 136, 247, 991, 2237, 5036, 8540\} 
%\{64, 247, 991, 5036, 8540\}
%corresponding to sampling 
%%\{10, 15, 20, 40, 60, 90, 120\} 
%\{10,  20, 40, 60,  120\} 
%logarithmically-spaced points for each T1 and T2 with T1$>$T2.
%
%%compare performance of \MCMRF by varying its storage requirement in the \todo{grid-search step (for initialising Blasso)} and considering grid-sizes \{64, 136, 247, 991, 2237, 5036, 8540\} corresponding to sampling \{10, 15, 20, 40, 60, 90, 120\} logarithmically-spaced points for T1 and T2 each, with T1$>$T2.
%
%
%\todo{be more clear about goals of this studty/expe}


%%======BLACKWHITE=====================
%%======BLACKWHITE=====================
%\begin{figure*}[ht!]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%
%\begin{turn}{90}  $\beta=0.0001$ \end{turn}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_21.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_22.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_23.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_24.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_25.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_26.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_27.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_28.pdf}
%\\
%\hspace{.3cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_29.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_210.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_211.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_212.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_213.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_214.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_215.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_216.pdf}\hspace{-.1cm}
%\\
%\vspace{.05cm}
%\hrule
%\hrule
%\vspace{.05cm}
%\begin{turn}{90} \, $\mathbf{\beta=0.001}$ \end{turn}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_31.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_32.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_33.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_34.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_35.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_36.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_37.pdf}\hspace{-.1cm}
%\\
%\vspace{.05cm}
%\hrule
%\hrule
%\vspace{.05cm}
%\begin{turn}{90} \quad $\beta=0.01$ \end{turn}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_51.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_52.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_53.pdf}\hspace{-.1cm}
%\qquad\quad
%\begin{turn}{90} \quad $\beta=0.05$ \end{turn}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_61.pdf}\hspace{-.1cm}
%\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_62.pdf}\hspace{-.1cm}
%\\
%\caption{{
%Estimated in-vivo compartments i.e. T1/T2s and mixture maps, using  
%\MCMRF (un-thresholded) for four values of $\beta$. 16 out of 25 compartments with highest energies are shown for $\beta=10^{-4}$, while for other $\beta$s all compartments are shown. Small $\beta$ values create fine-detailed decompositions whereas larger $\beta$ values hierarchically cluster compartments together.
%}\label{fig:vivo_fullmixtures} }
%\end{minipage}} 
%\end{figure*}


%======= COLORED
\begin{figure*}[ht!]
	\centering
	\scalebox{1}{
	\begin{minipage}{\linewidth}
		\centering		

\begin{turn}{90}  $\beta=0.0001$ \end{turn}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_21c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_22c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_23c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_25c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_24c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_26c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_27c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_28c.pdf}
\\
\hspace{.3cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_29c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_210c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_211c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_212c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_213c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_214c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_215c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_216c.pdf}\hspace{-.1cm}
\\
\vspace{.05cm}
\hrule
\hrule
\vspace{.05cm}
\begin{turn}{90} \, $\mathbf{\beta=0.001}$ \end{turn}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_31c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_32c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_33c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_34c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_35c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_36c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_37c.pdf}\hspace{-.1cm}
\\
\vspace{.05cm}
\hrule
\hrule
\vspace{.05cm}
\begin{turn}{90} \quad $\beta=0.01$ \end{turn}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_51c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_52c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_53c.pdf}\hspace{-.1cm}
\qquad\quad
\begin{turn}{90} \quad $\beta=0.05$ \end{turn}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_61c.pdf}\hspace{-.1cm}
\includegraphics[width=.12\linewidth]{../figs_gen/vivo/figs/expe13_im_62c.pdf}\hspace{-.1cm}
\\
\caption{{
Estimated in-vivo compartments i.e. T1/T2s and mixture maps, using  
\MCMRF (un-thresholded) for four values of $\beta$. 16 out of 25 compartments with highest energies are shown for $\beta=10^{-4}$, while for other $\beta$s all compartments are shown. Small $\beta$ values create fine-detailed decompositions whereas larger $\beta$ values hierarchically cluster compartments together.
}\label{fig:vivo_fullmixtures} }
\end{minipage}} 
\end{figure*}






\begin{figure*}[ht!]
	\centering
	\scalebox{1}{
	\begin{minipage}{\linewidth}
		\centering		
%\begin{turn}{90} \qquad PVMRF \end{turn}
\includegraphics[width=.24\linewidth]{../figs_gen/vivo/figs/expe1_scatter_2.pdf}
\includegraphics[width=.24\linewidth]{../figs_gen/vivo/figs/expe1_scatter_3.pdf}
%\includegraphics[width=.19\linewidth]{../figs_gen/vivo/figs/expe1_scatter_4.pdf}
\includegraphics[width=.24\linewidth]{../figs_gen/vivo/figs/expe1_scatter_5.pdf}
\includegraphics[width=.24\linewidth]{../figs_gen/vivo/figs/expe1_scatter_6.pdf}
\\
 \hspace{.5cm}  (a) \MCMRF $\beta=10^{-4}$ \hspace{.7cm} (b) \textbf{\MCMRF $\mathbf{\beta=10^{-3}}$} \hspace{.5cm} (c) \MCMRF $\beta=10^{-2}$ \hspace{.5cm} (d) \MCMRF $\beta=5\times10^{-2}$ \\
\vspace{.2cm}

%====== scatterplot compare baselines=====================	
%\begin{turn}{90} \qquad PVMRF \end{turn}
\includegraphics[width=.24\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_111.pdf}
\includegraphics[width=.24\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_121.pdf}
\includegraphics[width=.24\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_131.pdf}
\includegraphics[width=.24\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_141.pdf}
\\
 \hspace{-1.6cm}(e) PVMRF \hspace{2.7cm} (f) SPIJN \hspace{2.9cm} (g) BayesianMRF \hspace{1.5cm} (h) SG-Lasso\\
%\vspace{.1cm}
\caption{{The T1/T2 values of the estimated in-vivo brain compartments (un-thresholded) using (a-d)
\MCMRF 
for different parameters $\beta$, and (e-h) the MC-MRF baselines. All methods used LRTV reconstruction before mixture separation. Scatter points' radii are scaled by the $\ell_2$ norms of the mixture weights (maps) corresponding to the estimates T1/T2s. }
\label{fig:vivo_compareScatter} }
\end{minipage}}
\end{figure*}




%%===================================================
%\begin{figure*}[t]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%\begin{turn}{90} \quad \textbf{\MCMRF} \end{turn}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1521.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1522.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1523.pdf}
%\hspace{.2cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2521.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2522.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2523.pdf}
%\\
%\begin{turn}{90} \qquad PVMRF \end{turn}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1121.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1122.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1123.pdf}
%\hspace{.2cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2121.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2122.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2123.pdf}
%\\
%\begin{turn}{90} \quad\quad SPIJN \end{turn}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1221.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1222.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1223.pdf}
%\hspace{.2cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2221.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2222.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2223.pdf}
%\\
%\begin{turn}{90} \quad BayesianMRF \end{turn}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1321.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1322.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1323.pdf}
%\hspace{.2cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2321.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2322.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2323.pdf}
%\\
%\begin{turn}{90} \quad SG-Lasso \end{turn}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1421.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1422.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1423.pdf}
%\hspace{.2cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2421.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2422.pdf}\hspace{-.1cm}
%\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2423.pdf}
%\\
%(a) methods used LRTV reconstruction\hspace{3cm} (b) methods used SVD-MRF reconstruction
%\caption{{Estimated mixture maps and their T1/T2s for the WM, GM and CSF in-vivo brain compartments using MC-MRF baselines and \MCMRF at sequence length $T=1000$. Methods used (a) LRTV or (b) SVD-MRF reconstructions before mixture separation. 
%}\label{fig:vivo_compareMM} }
%\end{minipage}}
%\end{figure*}

%===================================================
\begin{figure*}[t]
	\centering
	\scalebox{1}{
	\begin{minipage}{\linewidth}
		\centering		
\begin{turn}{90} \quad \textbf{\MCMRF} \end{turn}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1521c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1522c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1523c.pdf}
\hspace{.2cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2521c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2522c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2523c.pdf}
\\
\begin{turn}{90} \qquad PVMRF \end{turn}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1121c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1122c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1123c.pdf}
\hspace{.2cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2121c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2122c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2123c.pdf}
\\
\begin{turn}{90} \quad\quad SPIJN \end{turn}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1221c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1222c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1223c.pdf}
\hspace{.2cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2221c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2222c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2223c.pdf}
\\
\begin{turn}{90} \quad BayesianMRF \end{turn}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1321c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1322c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1323c.pdf}
\hspace{.2cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2321c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2322c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2323c.pdf}
\\
\begin{turn}{90} \quad SG-Lasso \end{turn}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1421c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1422c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1423c.pdf}
\hspace{.2cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2421c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2422c.pdf}\hspace{-.1cm}
\includegraphics[width=.155\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2423c.pdf}
\\
(a) methods used LRTV reconstruction\hspace{3cm} (b) methods used SVD-MRF reconstruction
\caption{{Estimated mixture maps and their T1/T2s for the WM, GM and CSF in-vivo brain compartments using MC-MRF baselines and \MCMRF at sequence length $T=1000$. Methods used (a) LRTV or (b) SVD-MRF reconstructions before mixture separation. 
}\label{fig:vivo_compareMM} }
\end{minipage}}
\end{figure*}

%=====TABLE==============================
\begin{table*}[t!]
	%\vspace{0cm}
	\centering
	\scalebox{.98}{
		\begin{tabular}{c|ccccc|ccccc}
			\toprule[0.2em]
			\multicolumn{1}{c}{}&\multicolumn{5}{c}{T1 (ms)}&\multicolumn{5}{c}{T2 (ms)}  \\	
			\midrule[0.1em]		
			Tissue &{Literature} & \textbf{\MCMRF} & PVMRF & SPIJN & BayesianMRF & {Literature} & \textbf{\MCMRF} & PVMRF & SPIJN & BayesianMRF \\	
			
			
			\midrule[0.1em]		
				\midrule[0.1em]					
			WM &   $694-862^{\dag}$  & 804 & 774 & 914 & 821  		& $68-87^{\dag,*}$& 79& 79 & 92 & 77\\
			GM &    $1074-1174^*$ & 1073 & 931 & 1262 & 821 		& $87-103^{\dag,*}$   & 97 & 88 & 130& 82 \\
			CSF & $4000-4500^+$  &3057 & 4586  & 5388 & 4839	 &$2100-2300^+$ &1090 & 4000 & 4000& 4000\\
			\bottomrule[0.2em]
		\end{tabular}		}
		\caption{Estimated T1/T2 values for in-vivo brain compartments WM, GM and CSF at $T=1000$ using MC-MRF baselines and our \MCMRF\ algorithm, compared to the 1.5T literature values \cite{sled2001quantitative}$^{\dag}$ \cite{stanisz2005t1}$^{*}$ \cite{haacke1999magnetic}$^{+}$. All methods used LRTV reconstruction.}\label{tab:t1t2vivo}
	\end{table*}
%=======================================

\subsection{In-vivo brain experiment}
\label{sec:vivo}
To demonstrate feasibility of the proposed approach in vivo, sub-sampled MRF data was acquired from a healthy volunteer's brain with an informed consent obtained. Acquisition used a 1.5T GE HDxT scanner with 8-channel receive-only head RF coil, $230\times230$ mm$^2$ field-of-view with $230\times230$ pixels image size, 5 mm slice thickness, with the above-mentioned FISP MRF protocol. A variable density spiral trajectory was used to sample the k-space across time. 
%A total number of 377 spiral interleaves were used to cover 
The total number of spiral interleaves were 377. One spiral arm including 920 k-space locations was sampled at each TR/timeframe and this sub-sampled pattern was rotated for the next TR. 
%One spiral arm was used at each TR/timeframe, to measure 920 k-space locations. This pattern was rotated for the next TR. 
The overall acquisition window was \todo{?? ms} for 1000 timeframes. 

%Validations focused on separating mixtures arisen from the WM, GM and CSF tissue compartments of the healthy brain. The lipid and skin tissues from skull were removed (masked) from the reconstructed TSMIs to keep only the region containing the brain. \todo{Throughout when LRTV was used, it's parameter was $\la_{\text{LRTV}}=10^{-5}$.}

We first used this data to examine effects of the parameter $\beta$ in the SGTV norm~\eqref{sgtvnorm} on mixture separation using the \MCMRF algorithm. 
%Parameters $\beta$ plays a key role in separation quality of the mixture maps as it interpolates between Lasso and group Lasso regularisations. 
TSMIs were reconstructed using LRTV with $\la_{\text{LRTV}}=10^{-5}$. We then ran \MCMRF\ for different values of $\beta=\{1, 10, 100, 500\}\times10^{-4}$ at a fixed regularisation weight $\alpha=0.8$. The estimated compartments (T1/T2 values) are scatter plotted in Figures~\ref{fig:vivo_compareScatter}(a-d). Mixture maps of these compartments are also shown in Figure~\ref{fig:vivo_fullmixtures}.  
As can be observed in these figures, interpolating between two extreme cases of sparsity (i.e. $\beta \rightarrow 0 \,\,\text{or}\,\, 1$, corresponding to lasso or a group lasso type penalty) creates non-trivial solutions (compartments) that are separated across the T1/T2 values as well as their spatial mixture maps. For small $\beta$ values tissues are decomposed into spatially finer compartments (Figure~\ref{fig:vivo_fullmixtures}), while larger $\beta$ values hierarchically cluster the tissue compartments together around few T1/T2 values. %into higher levels of abstraction. % in a hierarchical fashion. 
% (with a possible bias in their estimated T1/T2s). 
Decompositions at a moderate value $\beta=10^{-3}$  indicates a  single component for WM, 
however for  GM and CSF (particularly in the boundaries) voxels can be decomposed into extra compartments with higher and lower relaxation times, correspondingly.

In our next experiment we used this data to compare the performance of \MCMRF\ with the MC-MRF baselines.
We used $\beta=10^{-3}, \alpha=0.8$ parameters for \MCMRF, and for visualisations the outcomes of all tested methods (baselines and ours) were hard thresholded to represent exactly three 
%most dominant 
compartments for WM, GM and CSF. For this the T1/T2 values of top two compartments with highest energy ($\ell_2$ norm) mixture maps were reported as WM and GM, 
%whereas for CSF (whose mixture map is sparse) 
and the longest 
%T1/T2 
compartment was reported as CSF.
%i.e. three rows of the normalised mixture map matrix $C_n$ with largest Euclidean norms. 
Given these T1/T2 estimates, the final mixture maps were computed (refined) through simulating a three-atom discrete dictionary and solving a small-sized nonnegative least squares for~\eqref{eq:model4}. %as in~\cite{SPIJN}.

Figure~\ref{fig:vivo_compareMM}(a) compares the mixture maps and the estimated T1/T2 resulted by \MCMRF\ and the baselines. 
%In Figure~\ref{fig:vivo_compareMM}(a) 
Here all methods used the LRTV reconstruction ($\la_\text{LRTV}=10^{-5}$) 
%and in Figure~\ref{fig:vivo_compareMM}(b) the SVD-MRF reconstructions 
before demixing step and the (post-processing) thresholding for visualising the WM, GM and CSF compartments. 
%In this figure comparisons are focused on WM, GM and CSF compartments. For this all regularisation algorithms follow the above-mentioned postprocesing step to hard threshold their results into final three compartments. PVMRF does not use this process because its k-means step already outputs hard thresholded results. 
In separate Figures~\ref{fig:vivo_compareScatter}(b,e-h) the T1/T2 values of all estimated compartments before thresholding are scatter plotted. Table~\ref{tab:t1t2vivo} compares the estimated T1/T2 values of tissues to their literature values at 1.5 Tesla. %Due to the in-vivo pulsation phenomenon~\cite{FISP} which is not modelled by the FISP sequence, MRF's CSF relaxations are not consistent with the literature and hence not included in this table. 
Table~\ref{tab:runtime} summarises runtimes of the tested MC-MRF algorithms.

%=====TABLE==============================
\begin{table}[t!]
	%\vspace{0cm}
	\centering
	\scalebox{1}{
		\begin{tabular}{ccccc}
			\toprule[0.2em]
			PVMRF & SPIJN & BayesianMRF & SG-Lasso & \MCMRF  \\	
			\midrule[0.05em]	
			\midrule[0.05em]		
			2.56& 220.91& 325.42& 	842.78 &102.30	\\
			\bottomrule[0.2em]
		\end{tabular}		}
		\caption{Runtimes (in seconds) of the MC-MRF algorithms for the in-vivo experiment.}
		\label{tab:runtime}
	\end{table}
%=======================================


In Figure~\ref{fig:vivo_compareMM}(a) \MCMRF\ outperforms baselines in terms of the visual appearance of the mixture maps, their spatial separability and correspondence to the anatomical structures of WM, GM and CSF. Further, the estimated T1/T2 values for both WM and GM are within the range of literature values~(see Table~\ref{tab:t1t2vivo}). Estimated CSF relaxations were lower than literature values due to the in-vivo pulsation phenomenon~\cite{FISP} that is not modelled by the MRF. Also note that the non-thresholded representation in Figure~\ref{fig:vivo_fullmixtures} suggests a range of long T1/T2 compartments (rather than a unique value) associated to the CSF.
BayesianMRF does not exploit group sparsity and results in many unclustered compartments (Figure~\ref{fig:vivo_compareScatter}(g)) and poor mixture maps. 
Baselines SPJIN and PVMRF improve this thanks to compartment grouping, however the WM map using SPJIN is not well separated from the GM region, and in PVMRF the GM map is not well separated from the CSF region (Figure~\ref{fig:vivo_compareMM}(a)). SPJIN overestimated the WM and GM's T1/T2 relaxations, BayesianMRF underestimated the GM's T1/T2  relaxations, PVMRF underestimated GM's T1 value, and all baselines overestimated the highest possible dictionary value for the CSF's T2. 
The non-iterative PVMRF was the fastest method, followed by \MCMRF\ which is the fasted amongst tested model-based iterative algorithms (Table~\ref{tab:runtime}). 
Notably, the (discretised) SG-Lasso implemented by FISTA at a high level of accuracy (objective tolerance=$10^{-8}$) and longest runtime, outputs unclustered (non-sparse) compartments (Figure~\ref{fig:vivo_compareScatter}(h)) and poor mixture maps (Figure~\ref{fig:vivo_compareMM}(a)), highlighting the significance of an off-the-grid alternative to overcome the fundamental limitation of sparse approximation in a highly coherent discretised dictionary. 

Figures~\ref{fig:vivo_compareMM}(b) show similar comparisons between MC-MRF methods where LRTV is replaced by the SVD-MRF~\cite{SVDMRF} (i.e. Fourier backprojection) reconstruction. Note that this is the method previously adopted by all baselines. 
%Reconstruction step influences mixture separation results and 
As can be observed, SVD-MRF produces undersampling artefacts that can propagate to the demixing step and hamper the results.  
These artefacts are less in the group-sparse methods PVMRF, SPIJN and \MCMRF\ for $T=1000$.
% show robustness against aliasing artefacts and \MCMRF\ outperforms baselines by producing more consistent mixture maps with those used LRTV in Figure~\ref{fig:vivo_compareMM}(a). 
 Additional results examining \MCMRF\ on truncated acquisition sequences 
 %$T=\{750,500,250\}$ 
 (supplementary materials, Figure~\ref{fig:vivo_cut_blasso}) highlight further the effectiveness of LRTV than SVD-MRF in short-length sequences ($T=750$ and $500$) for reducing mixture map errors, consistent with brain phantom results in Figure~\ref{fig:barinweb_boxchart}. 
Despite larger errors for CSF's relaxations,  here the WM and GM's T1/T2 estimations remained close to the literature values. % whereas the CSF's T2 showed increased underestimations for truncated  sequences.

%\todo{add something re for 750/500 things are good but 250 is too low. Also T2 of CSF is very sensitive which gets bad rapodily in smaller Ts,  estim get}









==> sections/model_old.tex <==
\section{Multi-compartment QMRI model}
Per-voxel magnetisation time-series signal $x\in \RR^T$ 
%$x \eqdef [x(t_1), x(t_2),\ldots, x(t_L)]^T$ 
resulted by multiple compartments follows a linear mixture model~\cite{BayesianPVMRF}:
\eql{\label{eq:model1}
x \approx \sum_s a_s \phi(\theta_s),
}
%\eql{\label{eq:model1}
%x \approx \Phi \meas \eqdef  \int \phi(\theta) \mathrm{d}\meas(\theta),
%}
where $\phi: \theta \in \Theta \rightarrow \RR^T$ denotes the Bloch magnetisation responses corresponding to the (unknown) latent NMR properties $\theta \in \Theta \subseteq \RR^d$.  The unknowns are the NMR properties $\ens{\theta_s}$ and the weights $\ens{a_s} \subset \RR_+$. 

%We denote by $\meas\in \Mm(\Theta; \RR_+)$ is an (unknown)  Radon measure defined on $\Theta$ \todo{write definition as footnote} i.e., the continuous domain of NMR properties, and it corresponds to the distribution of linear weights over $\theta$, according to which the corresponding magnetisation responses are mixed~\eqref{eq:model1}. 

We can consider a multi-dimensional extension of the above formulation for all $v$ voxels of the TSMI $X=[x_1,x_2,\ldots,x_v]\in\RR^{T \times v}$:
\eql{\label{eq:model2}
X \approx \sum_s \phi(\theta_s) c_s^\top
}
where $c_s\in\RR_+^v$  correspond to the $\theta$-dependent mixture weights for all voxels i.e. mixture map images. 


%through defining a vector-valued measure $\meas\in \Mm (\Theta; \RR_{+}^{1\times v})$:
%\eql{\label{eq:model2}
%X \approx \Phi \meas,
%}
%where (with slight abuse of notation) here $\meas$ corresponds to $\theta$-dependent mixture weights for all voxels i.e. mixture map images. 
%The goal is to approximate~\eqref{eq:model2} by a sparse measure of the following form  with few components in the summation:
%\eql{\label{eq:meas}
%\meas = \sum_s c^T_s {\delta}(\theta-\theta_s),
%}
%where $c_s\in \RR_{+}^{v}$ and $\delta(.)$ denotes Dirac's mass function. This implies \emph{sparse mixture factorisation} 
%\eql{\label{eq:model3}
%X \approx \sum_s \phi(\theta_s)c_s^T,
%}
%wherein the \emph{entire} TSMI voxels are decomposed into few compartments ($\theta_s$) and their corresponding mixture maps ($c_s$).

Previous works \nref have deal with the problem of recovering the NMR properties and mixture maps $\ens{\theta_s, c_s}$  by quantising the NMR properties space $\overline{\Theta}=[\Theta]$ \todo{what does $[\Theta]$ mean?} over a dense grid, and forming a combinatorially large MRF dictionary $D\eqdef\{\phi(\overline \theta)\}_{\forall \overline \theta \in \overline{\Theta}}$ of $d=\Card(\Theta)$ fingerprints. This has lead to the discretised/gridded formulation:
\eql{\label{eq:model4}
X \approx DC^\top,
}
where one aims to find a sparse (or a column-sparse) representation for the very large-sized matrix $C\in\RR_+^{v\times d}$ containing mixture maps for every possible fingerprint. Besides sparsity, the positivity of the mixture maps is observed an important constraint for rejecting spurious solutions to this ill-posed inverse problem (this could be traced in other QMRI works \nref beyond the MRF literature). 

\section{Sparse Group Beurling Lasso (SGB-Lasso)}
In this work, we consider a continuous approach by writing \eqref{eq:model2} as a continuous linear model over the space of finite vector-valued measures. First observe that  by writing
\eql{\label{eq:meas}
\meas = \sum_s c^T_s \delta_{\theta_s}
}
where $c_s\in \RR_{+}^{v}$ and $\delta_\theta$ denotes Dirac's mass function at position $\theta\in \Theta$, and defining a linear operator $\Phi$ over the space of vector valued measure $\Mm(\Theta;\RR^v)$ as
\eql{\label{eq:model3}
\Phi \meas \eqdef \int \phi(\theta) \mathrm{d}\meas(\theta),
}
equation \eqref{eq:model2} becomes $X = \Phi \meas$. We therefore consider the finite dimensional linear inverse problem of recovering an unknown measure $\meas$ from measurements $X$. Since we expect the underlying measure to be a sparse measure of the form \eqref{eq:meas} where each mixture map $c_s$ is itself sparse, we propose to solve \eqref{eq:model3} by the following variational formulation, coined as Sparse Group Beurling Lasso (SGB-Lasso)
\eql{\label{eq:spglasso}
\argmin_{\meas\in\Mm(\Theta;\RR_{+}^v)} \frac12 \norm{X - \Phi \meas}_{F}^2 + \alpha \norm{\meas}_{\beta}.
}
The regularisation parameter $\alpha\geq 0$ balances between a TSMI fidelity term and a sparsity-promoting norm.  We define the Sparse Group Total Variation (SGTV) norm $\|.\|_{\beta}$ though the following composition of variation norms for vector-valued measures: 
Given a vector-valued measure $\meas\in \Mm(\Theta; Y)$ taking values in a Banach space $Y$ endowed with norm $\norm{\cdot}_Y$, its variation is defined to be
$$
\abs{\meas}_Y(\Theta)  = \sup_{A_i} \sum_{i=1}^n \norm{\meas(A_i)}_Y
$$
where the supremum is over all partition $\ens{A_i}_{i=1}^n$ of $\Theta$. In our setting, $Y = \RR^v_+$ and by endowing this space with $\norm{c}_1 \eqdef \sum_{i=1}^v \abs{c_i}$ and $\norm{c}_2 \eqdef \sqrt{\sum_{i=1}^v \abs{c_i}^2}$, we denote the corresponding variations by $\abs{\meas}_1$ and $\abs{\meas}_2$, and define the group sparse regularisation norm as
$$
\norm{\meas}_{\beta} \eqdef \beta \abs{\meas}_1(\Theta) + (1-\beta) \sqrt{v} \abs{\meas}_2(\Theta).
$$
With respect to~\eqref{eq:meas} we have the identity \footnote{to be distinguished with Osher's TV. \todo{also add maths definitions for $\norm{\meas}_1$ and $\norm{\meas}_{1,2}$ possibly in the footnote}} 
\eql{\label{sgtvnorm}
\norm{\meas}_{\beta} =\sum_{s} \beta \norm{c_s}_{1} + (1-\beta)\sqrt{v} \norm{c_s}_{2}.
}
%The norm $\norm{\meas}_{1}$ norm promotes two types of sparsity: i) compartment-sparsity in a sense that few compartments  ($\theta_s$) 
%contribute to the TSMI across all voxels, as well as ii) mixture map sparsity in the sense that the mixture map/image ($c_s$) of each contributing compartment is spatially sparse. The addition of the second norm $\norm{\meas}_{1,2}$ weighted by $\beta$ 

Note that $\norm{.}_{\beta}$ is a continuous extension of the regularisation introduced in~\cite{SPGLasso} for discretised dictionaries. 
The term  $\abs{\meas}_{2}(\Theta)$ promotes \emph{group sparsity} in a sense that few compartments  ($\theta_s$)  should 
%(however with possibly dense mixture maps for each) 
contribute to approximate the entire TSMI across all voxels \eqref{eq:model3}.  The term $\abs{\meas}_{1}(\Theta)$ in addition promotes \emph{spatial sparsity} within the mixture map/image ($c_s$) of each contributing compartment i.e., a voxel should usually receive contributions from fewer compartments than those composing the entire TSMI\todo{related to voxel purity?}, which helps to improve cross-compartment spatial separability of the mixture maps.
The parameter $\beta$ provides a degree of freedom to balance between these forms of sparsity and decompose TSMI at a desired level of abstractions/details across the NMR properties as well as image voxels (see for example Figure~\ref{fig:vivo_fullmixtures}).

\section{Theoretical analysis: Identifiability of the mixtures via \MCMRF}
%\section{Theoretical guarantees  of mixture separation via \MCMRF}

Suppose now that $X = \Phi \meas + w$ where $\meas$ is a sparse measure of the form \eqref{eq:meas} and $w\in \RR^{T\times v}$ denotes additive noise. We assume that $\norm{w} \leq \epsilon$ for some $\epsilon>0$.  In this section, we present a condition under which  solutions of \eqref{eq:spglasso} have the same sparsity structure as $\meas$,  provided that $\epsilon$ and $\alpha$  are sufficiently small. We do so via analysis of the dual problem to \eqref{eq:spglassodual}.



 The adjoint operator  of $\Phi$ is $\Phi^*:\RR^{T\times v}\to \Cc(\Theta;\RR^v)$ maps into the space of continuous vector valued functions.  Given  $p \in\RR^{T\times v}$ with columns $p_i$, $\Phi^* p = (f_i)_{i=1}^v$ where
 $
 f_i(\theta) =
 \dotp{\phi(\theta)}{p_i}
 $.
Let $\Phi_\btheta^*$ be the matrix with rows $\phi(\theta_s)^\top$ for $s\in [k]$. For $p\in \RR^{T\times v}$, $\Phi_\btheta^* p \in \RR^{k\times v}$ and for $c\in \RR^{k\times v}$, $\Phi_\btheta c= \sum_{s=1}^k \phi(\theta_s) c_s^\top \in \RR^{T \times v}$.  Given $f:\RR^n\to \RR^m$, let $J_f(\theta) \in \RR^{m\times n}$ denote the Jacobian of $f$ at $\theta$. Given a matrix $p\in \RR^{n\times m}$, let $\vc(p)\in\RR^{nm}$ be its vectorized version, let $\rc$ be the inverse operation, so that $\rc(\vc(p)) = p$.
 
 \begin{lem}
 The dual problem to \eqref{eq:spglasso} is
 \eql{\label{eq:spglassodual}
\sup_{p\in K} \dotp{X}{p}_F - \alpha \norm{p}_F^2
}
where $K\subseteq \RR^{T\times v}$ is defined as
$$
K \eqdef 
\enscond{p}{\eta \eqdef \Phi^* p, \; \sum_{i=1}^v ({\eta_i(\theta)} - \beta )_+^2 \leq v(1-\beta)^2}
 $$
 The primal and dual problems are related by $\meas$ solves \eqref{eq:spglasso} if and only if $p= \frac{\Phi^* \meas - X}{\alpha}$ solves \eqref{eq:spglassodual}.  Moreover, 
  any solution $\meas_\alpha$ to \eqref{eq:spglassodual} satisfies
$$
\Supp(\meas_\alpha) \subseteq \enscond{\theta\in\Theta}{ \norm{f(\theta)} = 1  }
$$
where $f(\theta) \eqdef \frac{1}{\sqrt{v}(1-\beta)  }  (\eta(\theta) - \beta)_+$ and $\eta \eqdef \Phi^* p$.
 If  $\meas_\alpha = \sum_s c_s^\top \delta(\theta - \theta_s)$ is a discrete measure, then for each $s$, $\Supp(c_s) \subseteq \enscond{j \in [v]}{\eta_j(\theta_s) > \beta}$.
 \end{lem}
\begin{proof}
It is known from \cite{} that  for $\epsilon>0$,
\begin{align*}
&\enscond{u+v}{u,v\in\RR^d, \norm{u}_2 \leq \epsilon \nu, \norm{v}_\infty \leq (1-\epsilon) \nu} \\
&= \enscond{\xi\in \RR^d}{\norm{\xi}_\epsilon \leq \nu}
\end{align*}
where the so-called $\epsilon$-norm, defined as $\nu = \norm{\xi}_\epsilon$  is the unique $\nu>0$ such that
$$
\sum_i (\abs{\xi_i} - (1-\epsilon)\nu)_+^2 - (\epsilon \nu)^2 = 0.
$$
Therefore,
\begin{align*}
&\enscond{u+v}{u,v\in\RR^d_+, \norm{u}_2 \leq (1-\beta)\sqrt{v} , \norm{v}_\infty \leq  \beta } \\
&= \enscond{\xi\in \RR^d_+}{ \sum_i ( \xi_i - \beta)_+^2 \leq v(1-\beta)^2 }
\end{align*}
and
\begin{align*}
\norm{\meas}_{\beta} = 
\sup_{f\in\Kk}{\dotp{f}{\meas}}
\end{align*}
where $$\Kk = \enscond{ f\in \Cc(\Theta;\RR^v_+)}{ \forall \theta\in\Theta, \;  \sum_i ( f_i(\theta) - \beta)_+^2 \leq v(1-\beta)^2}.
$$
The result now follows by the Fenchel-Rockafellar duality theorem \cite{}.

\end{proof}


Note that \eqref{eq:spglassodual} has a unique solution, since it can be seen as the projection of $X/\alpha$ onto the closed convex set $K$.  Moreover, the previous lemma shows that its solution characterises the support of any primal solution $\meas$ of \eqref{eq:spglasso}. Therefore, to understand the structure of solutions to \eqref{eq:spglasso} with   $X = \Phi \meas + w$, it suffices to study the solution of the dual problem \eqref{eq:spglassodual}, which we denote by $p_{\alpha,\epsilon}$.

%\begin{lem}
%Let $p_\alpha$ solve \eqref{eq:spglassodual}. Then, letting $\eta_\alpha \eqdef \Phi^* p_\alpha$, any solution $\meas_\alpha$ to \eqref{eq:spglassodual} satisfies
%$$
%\Supp(\meas_\alpha) \subseteq \enscond{\theta\in\Theta}{ \sum_i (\eta_i(\theta) - \beta)_+^2 =v (1-\beta)^2  }
%$$
% and if $\meas_\alpha = \sum_s c_s^\top \delta(\theta - \theta_s)$ is a discrete measure, then for each $s$, $\Supp(c_s) \subseteq \enscond{j \in [v]}{\eta_j(\theta_s) > \beta}$.
%\end{lem}

Following \cite{}, we can show that $p_{\alpha,\epsilon}$ has a limit as $\epsilon/\alpha$ and $\alpha$ converge to 0:
Define the \textit{minimal norm certificate} by
\eql{
p_0 \in \argmin \enscond{\norm{p}_F}{  \eta \eqdef \Phi^* p, \; \sum_{i=1}^v ({\eta_i(\theta)} - \beta )_+^2 \leq v (1-\beta)^2 }
}
\begin{lem}
We have $\norm{p_{\alpha,0} - p_0}_F \to 0$ as $\alpha\to 0$, and
$$
\norm{p_{\alpha,\epsilon} - p_{\alpha, 0}} \leq \epsilon/\alpha.
$$
\end{lem}
\begin{proof}
\end{proof}



Define $\eta_0 \eqdef \Phi^* p_0$  and $f_0 \eqdef \frac{1}{\sqrt{v}(1-\beta)} (\eta_0 -\beta)_+$.
We say that $p_0$ is nondegenerate  with respect to a sparse measure $\meas_0 = \sum_{s=1}^k c_s \delta(\theta - \theta_s)$ 
satisfies 
\begin{enumerate}
\item $f_0(\theta)<1$ for all $\theta\not\in \ens{\theta_i}$
\item for each $s\in [k]$, $f(\theta_s) =  \frac{c_s}{\norm{c_s}_2}$.
\item  letting $g(\theta) \eqdef  \norm{f(\theta)}_2^2$, $g''(\theta_s) \neq 0$ for all $s\in [k]$. 
%and 
%$$
%\sum_{i\in \Supp(c_s)} ({\eta_i(\theta_s)} - \beta )_+\nabla^2 \eta_i(\theta) +\nabla \eta_i(\theta_s) [\nabla \eta_i(\theta_s) ]^\top <0
%$$
\end{enumerate}

\begin{prop}
If $p_0$ is nondegenerate, then provided that $\epsilon/\alpha$ and $\alpha$ are sufficiently small, the solution to \eqref{eq:spglasso} is of the form $\meas_{\alpha,\epsilon} = \sum_{j=1}^k \hat c_j \delta_{\hat \theta_j}$ where $\Supp(\hat c_j) \subseteq \Supp(c_j)$.
\end{prop}
\begin{proof}

Since $\norm{p_{\alpha,\epsilon}-p_{\alpha,0}} \leq  \norm{P_\Kk(X/\alpha) - P_\Kk((X+w)/\alpha)}  \leq \norm{w}_F/\alpha$, if $\eta_0$ is non-degenerate, then given any $r>0$, provided that $\norm{w}_F/\alpha$ and $\alpha$ are sufficiently small, letting $f(\theta) \eqdef \frac{1}{v (1-\beta)} \norm{(\eta_{\al,\epsilon}(\theta) - \beta)_+}^2 $, $f(\theta)<1$ for all $\theta \not\in \setminus \cup_j B_r(\theta_j)$, and for all $\theta\in B_r(\theta_j)$, $f''(\theta) \neq 0$. So, there are at most $k$ points for which $f(\theta) = 1$.  So, given data $X =\Phi \meas + w$, we recover at most $k$ components. Since $\eta_{\alpha,\epsilon}$ converges uniformly to $\eta_0$, it is also clear that $\meas_{\alpha,\epsilon} = \sum_{j=1}^k \hat c_j \delta_{\hat \theta_j}$ where $\Supp(\hat c_j) \subseteq \Supp(c_j)$.
\end{proof}


To establish support stability, it suffices to show that $p_0$ is nondegenerate. We look at the following proxy of $p_0$ which has a closed form expression: First note that the constraint $f_0(\theta_s) = \frac{c_s}{\norm{c_s}_2}$ for all $s\in [k]$ can be written as
\begin{align*}
P_{\bold{I}} \vc\pa{ \Phi^*_{\btheta} p_0}= P_{\bold{I}} [\Id_v \otimes \Phi_{\btheta}^*]\vc(p_0) = u_0
\end{align*}
where $u_0 = \pa{\beta + \sqrt{v}(1-\beta) P_{I_s}  c_s/\norm{c_s}_2}_{s=1}^k \in \RR^{kv}$ and given $Z=(Z_s)_{s=1}^k \in \RR^{k v}$, $P_{\bold{I}}(Z) =( P_{I_s} Z_s)_{s=1}^k$. Since $\norm{f_0(\theta)}^2 \leq 1$ for all $\theta$ and $\norm{f_0(\theta_s)}_2 = 1$, it is necessary that $\partial_\theta \norm{f_0(\theta_s)}_2^2 = 0$  for all $s\in [k]$, and hence,
\begin{align*}
0_d &= \sum_{i=1}^v (c_s)_i \nabla (\eta_0)_i(\theta_s) \\
&= J_\phi(\theta_s)^\top p_0 c_s =[ c_s^\top\otimes J_\phi(\theta_s)^\top]\vc(p_0)
\end{align*}
Defining the $Tv\times (\sum_{s=1}^k \abs{I_s}+kd)$ matrix $$\Gamma = [\Id_v\otimes \Phi_\btheta P_{\bold{I}}^* , c_1\otimes J_\phi(\theta_1), \cdots, c_k \otimes J_\phi(\theta_k)] $$
we see that $p_0$ must satisfy
$$
\Gamma^{*} p_0 = \begin{pmatrix}
u_0\\
0_{kd}
\end{pmatrix}.
$$
So, if $\eta_V \eqdef \Phi^* \rc \pa{(\Gamma^*)^\dagger \begin{pmatrix}
u_0\\
0_{kd}
\end{pmatrix}}$ satisfies $\norm{\eta_V(\theta)}_2 \leq 1$ for all $\theta$, then $\eta_V = \eta_0$ and we have a closed form expression for $\eta_0$. Note that by definition, $\eta_V(\theta_s) = \eta_0(\theta_s)$. 
\begin{defn}
We call  $\eta_V$ the vanishing derivatives precertificate and say that it is nondegenerate if $\eta_V(\theta) <1$ for all $\theta \not\in \ens{\theta_s}_{s=1}^k$ and $ g_V(\theta) \eqdef  \norm{\eta_V(\theta)}^2$ satisfies $g_V''(\theta_s) \neq 0$ for all $s\in [k]$.

\end{defn}
Clearly, if $\eta_V$ is nondegnerate, then $\eta_V = \eta_0$ is also nondegenerate.



\begin{thm}
Let $X = \Phi \meas_0 + \epsilon$ where $\epsilon \in \RR^{T\times v}$ satisfies $\norm{\epsilon}_F \leq \delta$ and $\meas_0 = \sum_{s=1}^k c_s \delta_{\theta_s}$. Suppose that $\Gamma$ is full rank and $\eta_0 \eqdef \Phi^* p_0$ is nondegenerate, then for all $\alpha$ and $\delta/\alpha$ sufficiently small,  \eqref{eq:spglasso} recovers a unique solution of the form $ \sum_{s=1}^k \tilde c_s \delta(\theta - \tilde \theta_s)$ with $\norm{\tilde c_s - c_s}_F \leq \delta$ and $\norm{\tilde \theta_s - \theta_s} \leq \delta$.

\end{thm}


%
%%\paragraph{Pre-certificate}
%Find $\eta = \Phi^* p$ with smallest $\norm{p}_F$  such that
%%$$
%%\frac{({\eta(\theta_s)} - \lambda_1 )_+}{\lambda_2} = \frac{c_s}{\norm{c_s}_2}
%%$$
%for each $s\in[k]$ and $I_s = \Supp(c_s)$,
%%$$
%%\frac{({\eta(\theta_s)} - \beta )_{I_s}}{\sqrt{v}(1-\beta)} = \frac{(c_s)_{I_s}}{\norm{c_s}_2}
%%$$
%$$
%\eta(\theta_s)_{I_s} = \beta 1_{I_s} +   \sqrt{v}(1-\beta) \frac{(c_s)_{I_s}}{\norm{c_s}_2}
%$$
%and
%$$
%\forall s\in [k], \qquad   \sum_{i=1}^v  (c_s)_i\nabla \eta_i(\theta_s) = 0
%$$
%If $\sum_{i=1}^v ({\eta_i(\theta)} - \beta )_+^2 \leq v(1-\beta)^2 $ for all $\theta\in\Theta$, then $\eta$ coincides with $\eta_0$.
%Note that $\eta$ can be computed numerically by solving a system of $\sum_{s=1}^k \abs{T_s} + k$ equations.
%
%Let $\Phi_\btheta^*$ be the matrix with rows $\phi(\theta_s)^\top$ for $s\in [k]$. Let $p\in \RR^{T\times v}$. So, $\Phi_\btheta^* p \in \RR^{k\times v}$, and we can rewrite the equations as
%\begin{align*}
%\diag(P_{I_s})_s \Phi_\btheta^* p = \pa{ \sqrt{v}(1-\beta) P_{I_s} \frac{(c_s)_{I_s}}{\norm{c_s}_2} + \beta }\\
%\forall s\in [k], \; J_\phi(\theta_s) p c_s = 0
%\end{align*}



\todo{We can do numerics to show that this precertificate is indeed nondegenerate for specific T1-T2 values}


\begin{proof}



Let $\meas_0 =  \sum_s (c_0)^\top_s {\delta}_{(\theta_0)_s}$.


%
%If $\meas = \sum_s c^\top_s {\delta}_{\theta_s}$ solves \eqref{eq:spglasso}, then, for each $s\in [k]$, denoting $I_s$ as the support of $c_s$,
%$$
%\eta \eqdef \frac{1}{\alpha} \Phi^*\pa{\Phi_{\btheta_0} c_0 + w - \Phi_\btheta c}
%$$
%we know that $$\eta(\theta_s)_{I_s} - \beta = \sqrt{v}(1-\beta) \frac{(c_s)_{I_s}}{\norm{c_s}}.
%$$ Since $\sum_{i=1}^v (\eta_i(\theta) - \beta)_+^2 \leq v(1-\beta)^2$ for  all $\theta\in\Theta$ with equality at each $\theta_s$, $s\in [k]$, we have for all $s\in [k]$,
%$$
%\partial_{\theta}
%\pa{\sum_{i=1}^v (\eta_i(\theta) - \beta)_+^2}(\theta_s) = 0.
%$$
%If follows that for all $s\in [k]$,
%$$
%\sum_{i=1}^v (\eta_i(\theta_s)-\beta)_+ \nabla \eta_i(\theta_s) = 0_{d}.
%$$
%Let $J_\phi(\theta) \in \RR^{T\times d}$ denote the Jacobian of $\phi$ at $\theta$, then observing that $(\eta(\theta_s)-\beta)_+ = c_s$, we have
%$$
%J_\phi(\theta)^\top \pa{\Phi_{\btheta_0} c_0 + w - \Phi_\btheta c} c_s = 0_d
%$$

Define a function
$$
F:\RR_+^{k\times v} \times \Theta^k \times \RR^{T \times v}\times  \RR_+ \to \RR^{\sum_{s=1}^k \abs{I_s} + kd}
$$
by $F(c,\theta,w,\lambda) = \begin{bmatrix}
\pa{g_i(c,\theta,w,\lambda)}_{i=1}^k\\
\pa{h_i(c,\theta,w,\lambda)}_{i=1}^k
\end{bmatrix}$
where writing $x\eqdef (c,\theta,w,\lambda)$,
$$
g_s(x) = P_{I_s}
\pa{ \phi(\theta_s)^\top[\Phi_\btheta c- \Phi_{\btheta_0} c_0- w ] + \lambda \pa{ \beta +  \sqrt{v} (1-\beta) \frac{c_s}{\norm{c_s}}}}
$$
and
$$
h_s(x) = J_{\phi}(\theta_s)^\top \pa{\Phi_\btheta c- \Phi_{\btheta_0} c_0- w} c_s
$$
Clearly, if $(c,\theta)$ correspond to a solution with data $y= \Phi_{\btheta_0} c_0 + w$, then $f(c,\theta,w,\lambda) = 0$. In particular, $f(c_0, \theta_0, 0,0) = 0$.

%Writing $u = (c,\theta)$, $\partial_u F(c_0,\theta_0,0,0) = \begin{pmatrix}
%A & B^*\\
%B & C
%\end{pmatrix} \in \RR^{n\times n}$ where $n = \sum_s \abs{I_s} + kd$, we have, denoting $\hat c_s = (c_s)_{I_s}$
%$$
%A_{s,\ell} =\pa{ \phi(\theta_s)^\top \phi(\theta_\ell) - \delta_{s,\ell} \lambda\sqrt{v}(1-\beta) \pa{\frac{1}{\norm{\hat c_\ell}_2} - \frac{\hat c_\ell \hat c_\ell^\top}{\norm{ c_\ell}^2}}}
%$$
%$$
%B_{s,\ell} = J_\phi(\theta_s) \phi(\theta_\ell) \hat c_s^\top \in \RR^{d \times \abs{I_s}}
%$$
%and
%$$
%C_{s,\ell} = J_{\phi}(\theta_s) J_{\phi} (\theta_\ell)^\top \hat c_\ell^\top\hat  c_s \in \RR^{d\times d}
%$$


Writing $u = (c,\theta)$, $\partial_u F(c_0,\theta_0,0,0) = \Gamma_{\btheta_0}^* \Gamma_{\btheta_0}$.
%
%$ \begin{pmatrix}
%A & B^*\\
%B & C
%\end{pmatrix} \in \RR^{n\times n}$ where $n = \sum_s \abs{I_s} + kd$, we have for $s,\ell\in [k]$,
%$$
%A_{s,\ell} = P_{I_s}\pa{ \phi(\theta_s)^\top \phi(\theta_\ell)\Id_{v\times v} } P_{I_v}
%$$
%$$
%B_{s,\ell} = J_\phi(\theta_s)^\top \phi(\theta_\ell)  c_s^\top P_{I_s} \in \RR^{d \times \abs{I_s}}
%$$
%and
%$$
%C_{s,\ell} = J_{\phi}(\theta_s)^\top  J_{\phi} (\theta_\ell) c_\ell^\top   c_s \in \RR^{d\times d}
%$$
By assumption, $\partial_u F$ is invertible. By the implicit function theorem, there exists neighbourhoods $U \subset \RR_+^{kv} \times \Theta^k$ of $(c_0, \theta_0)$ and $V\subset \RR^{Lv}\times \RR_+$ of $(0,0)$ and a unique  continuously differentiable function $g:V\to U$ such that $F(g(v), v) = 0$ for all $v = (w,\lambda)\in V$. Moreover, since $g$ is continuously differentiable, $\norm{g(v) - g(0)} \leq C \norm{v}$. In particular, writing $(c,\theta) = g(v)$,
$$
\norm{c - c_0}_F+ \norm{\theta - \theta_0} \leq C (\lambda + \norm{w}_F) .
$$
Finally,  by uniqueness, $g(v)$ coincides with solutions of \eqref{eq:spglasso}.
\end{proof}


\section{Algorithms}
\subsection{TSMI reconstruction} Prior to mixture separation, the TSMI is computed from subsampled k-space measurements using the LRTV algorithm~\cite[Eq(10)]{MRFLRTV}. This method is dictionary-matching-free and does not limit reconstruction accuracy to the finite resolution of a discretised MRF dictionary. By exploiting TSMI's spatiotemporal structures, LRTV can efficiency remove aliasing artefacts 
%in under-sampled k-space regimes 
and is shown more accurate than the Fourier backprojection scheme SVD-MRF~\cite{SVDMRF} used by most MC-MRF baselines. %~\cite{SPIJN,PVMRF,BayesianPVMRF}.  
%An attractive feature of LRTV (also SVD-MRF) is exploiting a low-rank subspace model for \emph{dimensionality-reduction} (see also~[zhao,ADMM,covertree]). For many MRF sequences, including FISP~\cite{FISP} in our experiments, the Bloch responses and TSMIs live in a low-dimensional subspace through the following factorisation:
LRTV (also SVD-MRF) exploits a low-rank subspace \emph{dimensionality reduction} for accelerated reconstructions. For many MRF sequences, including FISP~\cite{FISP} in our experiments, the Bloch responses and TSMIs can be factorised in a low-dimensional subspace: % through the following factorisation:
\eq{
%\forall \theta \in \Theta, \,\, 
\phi(.) \approx VV^T\phi(.)\,  \qandq X \approx VV^TX, 
}
where $V$ is a $T\times \tau$ tall matrix representing the subspace of dimension $\tau\ll T$. %Working with 
%This  representation greatly accelerates %facilitates computations during 
%TSMI reconstruction (as well as solving the MC-MRF problem). 
%via \MCMRF where in \eqref{eq:spglasso} $X$ and $\phi(.)$ are replaced by the compressed TSMI $V^TX$ and compressed Bloch responses $V^T\phi$, respectively.
The raw TSMIs (complex-valued) are then \emph{phase-corrected} and mapped to real-valued images before being fed to the mixture separation step. This is particularly important for imposing the positivity constraint in~\eqref{eq:model2} and \MCMRF. For FISP sequence with constant TE per-voxel signal evolution has a constant complex-valued phase~\cite{SPIJN,FISP}. This  phase can be estimated from the first (principal) image component of the dimension-reduced TSMI and removed from the image~\cite{AIRMRF, coverblip_iop, MRFLRTV}. 

\subsection{Solving \MCMRF by Frank-Wolfe iterations}
 \todo{by clarice}
To solve this, we apply the following algorithm, which is an application of the Frank-Wolfe algorithm with nonconvex updates. Let $\theta^0 = []$, $c^0 = []$.  For each $k=0,1,2,\ldots$, 
\begin{enumerate}
\item Define  $\meas^k = \Phi_{\btheta^k}c^k$ and $\eta^k = \Phi^* (X-\Phi \meas^k)/\alpha$
\item Terminate if $\sup_{\theta\in\Theta}\sum_{i=1}^v (\abs{\eta^k_i(\theta)} - \lambda_1 )_+^2 \leq \lambda_2^2$.
\item  Let $\theta \in  \argmax_{\theta\in\Theta} 
     \sum_{i=1}^v \pa{  \eta^k(\theta)_i - \lambda_1}_+^2$
\item $c^{k+\frac12} \in \argmin_{c\in\RR_+^{k\times v}}\frac12 \norm{X- \Phi_{\btheta^{k+\frac12}}  c }_F^2 + \alpha \pa{\lambda_1 \norm{c}_1 + \lambda_2 \norm{c}_{1,2}}$
\item Initialising with $c^{k+1/2}$ and $\theta^{k+1/2}$, use LBFGS to solve $(c^{k+1},\theta^{k+1}) \in \argmin_{\theta,c} \frac12 \norm{X- \Phi_{\btheta^{k+\frac12}}  c }_F^2 + \alpha \pa{\lambda_1 \norm{c}_1 + \lambda_2 \norm{c}_{1,2}}$.
\end{enumerate}
\marginpar{\tiny{Issue with 5: BFGS does not solve nonsmooth L1. Signs where rather used in our code. Also, must be $\Phi_\theta$ not $\Phi_\theta^{k+.5}$ }}




\todo{Move the derivation of the algorithm to the appendix?}
The Frank-Wolfe algorithm seeks to solve minimisation problems of the form 
$$
\min_{m\in C} F(m)
$$
where $f:X\to \RR$ is a continuously differentiable function defined on some Banach space $X$, and $C\subseteq X$ is a bounded convex  set. To  derive our algorithm, we follow \cite{} by rewriting \eqref{eq:spglasso} as the minimisation of a differentiable function over a bounded convex set. Note that  the optimal measure satisfies
$$
\frac12 \norm{\Phi \meas - X}_F^2 +  \lambda_1 \norm{\meas}_{1}  + \lambda_2 \norm{\meas}_{1,2} \leq \norm{X}_F^2/2
$$
So in particular, $\norm{\meas}_{1} \leq \norm{X}_F^2/\pa{2\lambda_1}$. We can therefore equivalently write this as
\begin{align*}
\min_{\meas\in\Mm_+(\Theta;\RR^p), t_1,t_2\in\RR} F(t_1,t_2,\meas) \eqdef \lambda_1 t_1 + \lambda_2 t_2 + \frac12 \norm{\Phi\meas - y}^2
\\
\qquad \text{subject to } (t_1,t_2,\meas)\in \Cc
\end{align*}
where $\Cc\eqdef \enscond{(t_1,t_2,\meas)}{\norm{\meas}_1 \leq t_1,  \norm{\meas}_{1,2}\le t_2,  t_2 \leq t_1 \leq \frac{\norm{X}_F^2}{2\lambda_1}}$.
The differential of $F$ is a bounded linear operator on $\RR\times \RR \times \Mm_+(\Theta;\RR^p)$. Writing $s \eqdef (t_1,t_2,\meas)$ and $s' \eqdef (t_1',t_2',\meas')$, we have  
$$
[\mathrm{d}F(s)]s' = \lambda_1 t_1' + \lambda_2 t_2' + \int [\Phi^*( \Phi \meas - y)] (\theta) \mathrm{d}\meas'(\theta)
$$
The Frank-Wolfe algorithm is an iterative algorithm consisting of the following two steps: Denoting the $k$th iterate by $m^k$, do
\begin{enumerate}
\item $
s^{k} \in \argmin_{s\in\Cc} \mathrm{d}F(m^k)(s)
$
\item $m^{k+1} = (1-\gamma_k) s^{k} +\gamma_k m_k$
\end{enumerate}
For the first step, we can restrict the minimisation to the the extremal points of the convex set $\Cc$, which are of the form $(\norm{M}_1, \norm{M}_2, M \delta_\theta)$ where $\theta\in \Theta$ and $M\in \RR_+^p$. Therefore, writing $m^k = (t_1,t_2,\meas^k)$, we are led to solve
\begin{equation}\label{eq:tosolve}
(\theta,M) \in \argmin_{\theta\in\Theta, M\in \RR^p_+}   \lambda_1 \norm{M}_1 + \lambda_2 \norm{M}_2 - \dotp{M}{\eta^k(\theta) }, 
\end{equation}
where $ \eta^k\eqdef -\Phi^*( \Phi \meas^k - y)$.
Let the optimal points be $M = (m_j)_{j=1}^p$ and $\theta$, then the optimality condition reads
$$
-\eta^k(\theta)_j + \lambda_2 \frac{m_j}{\norm{M}_2} + \lambda_1 = 0, \qquad \text{ if } m_j >0
$$
$$
\eta^k(\theta)_j \in [0, \lambda_1], \qquad \text{ if } m_j =0
$$
i.e. we have 
$$
  \frac{M}{\norm{M}_2} = \frac{1}{\lambda_2} \pa{  \eta^k(\theta) - \lambda_1}_+
$$
Plugging this back into \eqref{eq:tosolve} and simplifying, we are left with
\begin{align}
\theta \in  \argmax_{\theta\in\Theta} 
     \sum_{i=1}^p \pa{  \eta^k(\theta)_i - \lambda_1}_+^2
\end{align}
The second step of the algorithm can be replaced by any procedure which improves the objective value.

%=================================
\begin{algorithm}[t!]
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} TSMI $X$, Bloch model $\phi(.)$, params $\alpha,\beta>0$.
\STATE \textbf{Outputs:} NMR parameters $\theta$, mixture weights $c$.
\STATE \textbf{Initialise:}  $\theta^0=\{\}$, $c^0=\{\}$.
\STATE \todo{@Clarice, moving FW steps here?}
\end{algorithmic}
\caption{\label{alg:FW} Frank-Wolfe iterations to solve \MCMRF~\eqref{eq:spglasso} } 
\end{algorithm}
%=========================================================	

\subsubsection{Nonconvex steps}
The Frank-Wolfe Algorithm~\ref{alg:FW} (steps 3 and 5) optimises nonconvex objectives (due to the nonlinearity of the Bloch responses) with respect to the NMR parameters $\theta$. We use the L-BFGS algorithm~\nref[paper+becker's code] to locally solve these steps. Step 3 is initialised by a coarse \emph{grid-search} over a small set of discretised NMR parameters $\overline{\Theta}$ i.e. a coarsely gridded dictionary used for enumerating $\eta^k(\theta)$,  $\forall \theta\in \overline{\Theta}$. Step 5 is initialised by the outcomes of the steps 3 and 4 for the NMR parameters and mixture weights, correspondingly. 

\subsubsection{Convex step}  \todo{} Algorithm~\ref{alg:FW} recovers one NMR compartment $\theta^\star$ per iteration, simulates its Bloch response and adds it to a dictionary $D\leftarrow D\cup \phi(\theta^\star)$. In step 4, $D$ is used for a discrete sparse group lasso problem~\cite{SPGLasso} solved by the fast shrinkage algorithm, FISTA. The shrinkage operator reads~\cite{SPGLasso}:
\eql{
\text{Prox}_{\lambda_1 \norm{.}_1 + \lambda_2 \norm{.}_{1,2}}(c) =
} 
Note that $D$'s size is small because Frank-Wolfe Algorithm is guaranteed to not iterate forever (in practice/numerical results, we maximum iterations to 30 while iterations were convergent earlier). Since $D$ is small, FISTA encounters no numerical issues and runs fast. 


\subsubsection{Neural network approximation}
%The Franke-Wolfe Algorithm~\nref[Pseudo-code] (steps 3 and 5) optimises nonconvex objectives (due to the nonlinearity of the Bloch responses) with respect to the NMR parameters $\theta$. We use the L-BFGS algorithm~\nref[paper+becker's code] to locally solve these steps.
Solving steps 3 and 5  requires computing derivatives of the Bloch responses with respect to the NMR parameters i.e. the jacobian matrix $\partial \phi(\theta)/\partial \theta$. 
While this can be analytically computed for simple forms of Bloch responses (e.g. MRF sequences in~\cite{dong2019quantitative,sbrizzi2017dictionary}, or the exponential models in 
classical quantitative MRI), such approach would not extent to more general non-analytical response models e.g. those like FISP simulated by the Extended Phase Graph (EPG) formalism~\cite{EPGWeigel}.
%When Bloch responses have simple recurrent formulations e.g. IR-bSSFP sequence~\cite{dong2019quantitative}, this can be done analytically despite long computations scaled by the sequence length $T$. However generally for non-analytical Bloch responses e.g. FISP sequence, this approach is not feasible. 
To circumvent this issue, we leverage on universal approximation property of neural networks~\cite{cybenko1989,lecun2015deep} that enables embedding complicated functions in conveniently differentiable surrogates via back-propagation mechanism. This idea is widely used in computer vision~\nref and physics~\nref, and was recently applied to single-compartment MRF reconstruction~\cite{PGDNET-MRF}. We train a neural network $\widetilde{\phi}: \theta\in\Theta \rightarrow \RR^{\tau} $ to approximate dimension-reduced Bloch responses (see section~\ref{sec:expe_neural} for more details). 
%i.e. $\widetilde{\phi}(\theta)\approx V^T\phi(\theta)$. 
This idea greatly accelerates Algorithm~\ref{alg:FW} i.e. in steps requiring function evaluation and differentiating Bloch responses: for solving 
%the MC-MRF problem via \MCMRF where in 
\eqref{eq:spglasso}, $X$ and $\phi(.)$ are replaced by 
%the compressed TSMI $\widetilde{X}\approx V^TX$ and neural approximate of the compressed Bloch responses $\widetilde{\phi}(\theta)\approx V^T\phi(\theta)$, respectively.
\eq{
\widetilde{X}\approx V^TX \qandq \widetilde{\phi}(\theta)\approx V^T\phi(\theta)
}
i.e. 
the compressed TSMI and neural approximate of the compressed Bloch responses, respectively.

%We therfore adopt a neural approach that a) facilitate dimension-reduction to accelerate computions  






==> sections/results.tex <==
\section{Results}

\subsection{Simulated data}
Subsampled k-space measurements from simulated brain data were corrupted by noise at different SNR levels and were fed to the \MCMRF\ algorithm for mixture separation. %using different grid sizes
Figure~\ref{fig:phan_noisegrid} reports the Mean Absolute Percentage Errors (MAPE) for estimating T1/T2 values of WM, GM and CSF compartments when \MCMRF\ used different grid sizes. Errors are averaged over 10 independent trials. \MCMRF's performance is robust to noise and grid-size: except the sensitive case of CSF's T2 at 20dB SNR, in other noise and grid-size regimes compartments were reliably recovered with average MAPEs less than $5\%$. 

Table~\ref{tab:expe_simul} compares \MCMRF\ and PVMRF baseline when both using LRTV reconstruction.  The T1/T2 MAPE (\%) errors and the mixture maps' SSIM and PNSR (dB) for estimating WM, GM, CSF compartments are reported for different acquisition lengths $T$ and non-exactly sparse (Gaussian-distributed) compartments $r$. Values are averaged over 10 Monte-Carlo runs of the experiments. Figures~\ref{fig:brainweb_SGBlasso} and~\ref{fig:brainweb_PVMRF} show an example of recovered compartments (T1/T2 values) and their mixture maps using \MCMRF and PVMRF methods, respectively. \todo{to be continued}



%%=======noise grid
%\begin{figure}[t]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%%\begin{turn}{90} \qquad PVMRF \end{turn}
%\includegraphics[width=.49\linewidth]{../figs_gen/brainweb/figs_expe1_noisegrid/plt_11.pdf}
%\includegraphics[width=.49\linewidth]{../figs_gen/brainweb/figs_expe1_noisegrid/plt_12.pdf}\\
%\includegraphics[width=.49\linewidth]{../figs_gen/brainweb/figs_expe1_noisegrid/plt_21.pdf}
%\includegraphics[width=.49\linewidth]{../figs_gen/brainweb/figs_expe1_noisegrid/plt_22.pdf}\\
%\includegraphics[width=.49\linewidth]{../figs_gen/brainweb/figs_expe1_noisegrid/plt_31.pdf}
%\includegraphics[width=.49\linewidth]{../figs_gen/brainweb/figs_expe1_noisegrid/plt_32.pdf}\\
%\caption{{MAPE errors for estimating T1/T2 values of WM, GM, CSF on simulated brain data, using \MCMRF\ with different grid sizes. Sub-sampled k-space measurements with different SNRs were fed to \MCMRF\ using different grid sizes. Errors are averaged over 10 independent trials for each SNR.}\label{fig:phan_noisegrid} }
%\end{minipage}}
%\end{figure}



%%=======	
%
%\begin{table*}[t!]
%	%\vspace{0cm}
%	\centering
%	\fontsize{9}{9}\selectfont
%	\scalebox{.8}{
%		\begin{tabular}{c|c|ccc|ccc|ccc}
%			\toprule[0.2em]
%			\multicolumn{2}{c}{} &\multicolumn{3}{c}{WM} & \multicolumn{3}{c}{GM} & \multicolumn{3}{c}{CSF}\\
%			\midrule[0.1em]
%%			\multicolumn{1}{c}{} &\multicolumn{2}{c}{MAPE (\%)} & \multicolumn{2}{c}{MAE (ms)} & \multicolumn{2}{c}{SNR (dB)} & \multicolumn{3}{c}{SSIM}  &  \multicolumn{2}{c}{MAPE (\%)} & \multicolumn{2}{c}{MAE (ms)} & \multicolumn{2}{c}{SNR (dB)} &\multicolumn{3}{c}{SSIM}  \\
%%			\midrule[0.1em]
%			&{$(T,r)$}&  {T1/T2 MAPE} &{PSNR} & {SSIM} &   {T1/T2 MAPE} &{PSNR} & {SSIM} & {T1/T2 MAPE} &{PSNR} & {SSIM}  \\
%			\midrule[0.05em]
%			\midrule[0.05em]
%			{\MCMRF} & \multirow{2}{*}{$(1000,0)$}& $5.33/2.23$ & $24.17$ & $0.855$ & $0.30/1.59$ & $23.29$& $0.934$ & $1.97/2.99$ & $36.62$ & $0.957$\\
%			%\midrule[0.05em]
%			{PVMRF} & & $ 4.65/2.18$ & $23.46$ & $0.845$ & $3.49/2.62$ & $18.07$ & $0.819$ & $25.49/38.48$ & $25.81$ & $0.810$ \\
%			\midrule[0.1em]
%			
%			{\MCMRF} & \multirow{2}{*}{$(500,0)$}& $5.02/3.04$ & $21.26$ & $0.805$ & $0.60/0.45$ & $19.62$  & $0.889$ & $0.22/21.34$ & $32.00$ & $0.921$ \\
%			%\midrule[0.05em]
%			{PVMRF} & & $3.96/2.85$ & $23.18$& $0.870$ & $2.44/3.17$ & $15.46$ & $0.777$ & $40.80/55.33$ & $19.69$ & $0.660$\\
%			
%			\midrule[0.1em]
%			{\MCMRF} & \multirow{2}{*}{$(250,0)$}& $3.53/9.03$ & 20.85 & 0.819 & $12.26/4.28$ & 21.81 & 0.928 & $26.70/47.38$ & 33.65 & 0.833 \\
%			%\midrule[0.05em]
%			{PVMRF} & & $3.63/11.9$ & $19.47$ & $0.777$ & $23.35/10.12$ & $20.16$ & $0.877$ & $18.20/44.59$ &  $33.31$ & $0.834$ \\
%			\midrule[0.1em]
%			{\MCMRF} & \multirow{2}{*}{$(1000,0.5)$}& $4.57/2.78 $& $21.59$ & $0.794$ & $1.05/1.36$ & $21.07$ & $0.911$ & $2.72/7.13$ & $32.58$ & $0.940$\\
%			%\midrule[0.05em]
%			{PVMRF} & & $4.33/2.93$ & $20.52$ & $0.797$ & $4.71/3.67$ & $13.74$ & $0.716$ & $42.90/60.63$ & $19.38$ & $0.711$ \\
%			\midrule[0.1em]
%			{\MCMRF} & \multirow{2}{*}{$(1000,1.0)$}& $4.43/4.80$ & 17.68 & 0.725 & $1.25/1.39$ & 17.44 & 0.846 & $11.76/28.96$ & 26.89 & 0.936\\
%			%\midrule[0.05em]
%			{PVMRF} & & $4.14/4.13$ & 18.97 & 0.786 & $4.17/2.55$ & 11.57 & 0.662 & $61.26/88.17$ & 14.45 & 0.606\\
%			\midrule[0.1em]
%			
%			{\MCMRF} & \multirow{2}{*}{$(1000,2.0)$}&$ 5.04/10.78$ & 12.07 & 0.628 & $0.51/3.28$ & 11.93 & 0.679 & $17.99/48.12$ & 20.57 & 0.834\\
%			%\midrule[0.05em]
%			{PVMRF} & & $4.43/9.11$ & $14.85$ & $0.687$ & $5.13/4.07$ & $10.79$ & $0.618$ & $77.11/99.71$ & $11.57$ & $0.509$\\
%			\midrule[0.1em]
%
%			
%		\bottomrule[0.2em]
%		\end{tabular}}
%		\caption{ The T1/T2 MAPE (\%) errors and the mixture maps' SSIM and PNSR (dB) using \MCMRF\ and PVMRF methods (both using LRTV reconstruction) for estimating WM, GM, CSF compartments in simulated brain, for different acquisition lengths $T$ and non-exactly sparse (Gaussian-distributed) compartments $r$. Values are averaged over 10 Monte-Carlo runs of the experiments.\todo{add std, besides MAPE ass actual t1/t2 values, add TSMI fidelity}} \vspace{.3cm}\label{tab:expe_simul}
%	\end{table*}
	
	
%\begin{figure}[t]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%\begin{turn}{90} \qquad $(1000,0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_1151.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_1152.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_1153.pdf}
%\\
%\begin{turn}{90} \qquad $(500,0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_3151.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_3152.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_3153.pdf}
%\\
%\begin{turn}{90} \qquad $(250,0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_4151.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_4152.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_4153.pdf}
%\\
%\begin{turn}{90} \qquad $(1000,0.5)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_1151.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_1152.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_1153.pdf}
%\\
%\begin{turn}{90} \qquad $(1000,1.0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_2151.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_2152.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_2153.pdf}
%\\
%\begin{turn}{90} \qquad $(1000,2.0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_3151.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_3152.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_3153.pdf}
%\caption{{The estimated T1/T2 values and the (normalised) mixture maps of the WM, GM and CSF compartments using \MCMRF at various $(T,r)$ values for sequence length $T$ and non-exact sparsity factor $r$. All methods used LRTV reconstruction before mixture separation. 
%}\label{fig:brainweb_SGBlasso} }
%\end{minipage}}
%\end{figure}
%
%
%\begin{figure}[t]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%\begin{turn}{90} \qquad $(1000,0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_1111.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_1112.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_1113.pdf}
%\\
%\begin{turn}{90} \qquad $(500,0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_3111.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_3112.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_3113.pdf}
%\\
%\begin{turn}{90} \qquad $(250,0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_4111.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_4112.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe3_cut/expe3_cut_im_4113.pdf}
%\\
%\begin{turn}{90} \qquad $(1000,0.5)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_1111.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_1112.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_1113.pdf}
%\\
%\begin{turn}{90} \qquad $(1000,1.0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_2111.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_2112.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_2113.pdf}
%\\
%\begin{turn}{90} \qquad $(1000,2.0)$ \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_3112.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_3111.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/brainweb/figs_expe2_GMM/expe2_GMM_im_3113.pdf}
%\caption{{The estimated T1/T2 values and the (normalised) mixture maps of the WM, GM and CSF compartments using PVMRF baseline at various $(T,r)$ values for sequence length $T$ and non-exact sparsity factor $r$. All methods used LRTV reconstruction before mixture separation. \todo{this figure stills shows unstability of PVMRF, why (250,0) should be better than (500,0) or (1000,0)?}
%}\label{fig:brainweb_PVMRF} }
%\end{minipage}}
%\end{figure}


	
	
\subsection{In vivo data}

Parameters $\beta$ plays a key role in separation quality of the mixture maps. It interpolate between lasso and group lasso. 
To examine this we used non-truncated FISP acquisition and chose values $\beta=\{1, 10, 100, 500\}\times10^{-4}$ for fixed $\alpha=0.8,\la=10^{-5}$. Estimated compartments (T1/T2 values) using \MCMRF\ are scatter plotted in Figure~\ref{fig:vivo_fullmixtures_scatter}, Mixture maps of these compartments are also shown in Figure~\ref{fig:vivo_fullmixtures}. Interpolating between two extreme cases of sparsity (i.e. $\beta \rightarrow 0 \qandq 1$) creates non-trivial solutions that are separated across the T1/T2 values as well as their spatial mixture maps. For small $\beta$ values tissues are decomposed into finer (more detailed) compartments, while larger $\beta$ values hierarchically cluster the tissues/compartments together. %into higher levels of abstraction. % in a hierarchical fashion. 
% (with a possible bias in their estimated T1/T2s). 
Decompositions at a moderate value $\beta=10^{-3}$  indicate a  single component for WM, 
however for  GM and CSF (particularly in the boundaries) voxels can be decomposed into extra compartments with higher and lower relaxation times, correspondingly.

%===== Hierachical clustering=========

%\begin{figure*}[ht!]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%				
%%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_11.pdf}
%%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_12.pdf}
%%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_13.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_21.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_22.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_23.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_24.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_25.pdf}
%%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_26.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_27.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_28.pdf}
%\\
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_31.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_32.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_33.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_34.pdf}
%%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_35.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_36.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_37.pdf}
%\\
%
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_41.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_42.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_43.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_44.pdf}
%\\
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_51.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_52.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_53.pdf}
%%\includegraphics[width=.17\linewidth]{../figs_gen/vivo/figs/expe1_im_54.pdf}
%\\
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_61.pdf}
%\includegraphics[width=.11\linewidth]{../figs_gen/vivo/figs/expe1_im_62.pdf}
%%\includegraphics[width=.17\linewidth]{../figs_gen/vivo/figs/expe1_im_63.pdf}
%%\includegraphics[width=.17\linewidth]{../figs_gen/vivo/figs/expe1_im_64.pdf}
%\\
%\caption{{
%The estimated T1/T2 values and normalised mixture maps using  
%\MCMRF\ prior to the post-process thresholding for (top to bottom) $\beta=\{1, 10, 100, 200,500\}\times10^{-4}$.
%}\label{fig:vivo_fullmixtures} }
%\end{minipage}}
%\end{figure*}
%




Figure~\ref{fig:vivo_compareMM} compares mixture maps and estimated T1/T2 resulted by \MCMRF and the MC-MRF baselines. All methods used LRTV reconstruction ($\la=10^{-5}$) before demixing step. In this figure comparisons are focused on WM, GM and CSF compartments. For this all regularisation algorithms follow the above-mentioned postprocessing step to hard threshold their results into final three compartments. PVMRF does not use this process because its k-means step already outputs hard thresholded results. 
In a separate Figure~\ref{fig:vivo_compareScatter} the T1/T2 values of all estimated compartments before thresholding are scatter plotted. 
\MCMRF\ and its discretised variant SG-Lasso used $(\alpha=0.8, \beta=10^{-3})$  parameters. BayesianMRF's parameters were $(\alpha_{\text{By}}=1.75, \beta_{\text{By}}=0.1, \mu_{\text{By}} = 10)$, and SPIJN's parameter was $\lambda_\text{Sp}=0.7$. 
\MCMRF\ used only 64 fingerprints for initialisation, whereas other methods used the complete MRF dictionary with 8’540 atoms. 

From Figure~\ref{fig:vivo_compareMM} we can observe \MCMRF\ outperforms all baselines in terms of the visual appearance of the mixture maps, their spatial separability and correspondence to the anatomical structures of WM, GM and CSF. Further, estimated T1/T2 values indicate close proximity to the literature values range for these tissues at 1.5T. \todo{add table or cite, also say T2 CSF is possibly under-estimated}. Remarkably, the (discretised) SG-Lasso implemented by FISTA at a fairly high level of accuracy (objective tolerance=1e-8), outputs inferior results, highlighting the significance of adopting the off-the-grid approach to overcome fundamental limitations of sparse approximation in highly coherent dictionaries. 

Figures~\ref{fig:vivo_compareMM2} and \ref{fig:vivo_compareScatter2} show similar comparisons  between MC-MRF methods when LRTV is replaced by SVD-MRF~\cite{SVDMRF} (i.e. Fourier backprojection) reconstruction. 
Note that this is the method that was originally adopted by all the baselines. 
Reconstruction  step influences mixture separation results and as can be observed, a less acurate reconstruction scheme can produce strong undersampling artefacts that propagate to demixing step and produce errors. 
Notably, group sparse methods PVMRF, SPIJN and \MCMRF\ show good robustness against aliasing artefacts of SVD-MRF. Remarkably \MCMRF outperforms baselines here and produces consistent maps with those reconstructed by LRTV in Figure~\ref{fig:vivo_compareMM} . \todo{say something about predicted T1/T2 values..how are they influenced?}



%BayesianMRF does not use group sparsity penalty and thus produces inferiorr results to  group methods PVMRF and SPIJN.  SPIJN does not fail like SPG-lasso because it has a pruning step. 

We also compared the performance of the proposed algorithm to the closest competitors PVMRF and SPIJN on shorter acquisition sequences truncated at $T=\{750, 500, 250\}$ timepoints. Figures~\ref{fig:vivo_cut_lrtv} and \ref{fig:vivo_cut_zf} show the results when LRTV and SVD-MRF reconstructions were used respectively prior to demixing. To clean aliasing artefacts, the LRTV's regularisation parameter was increased $\la=\{1,2,4\}\times 10^{-5}$ as the sequence was truncated shorter. \todo{upto 750 and 500 \MCMRF works reasonably well with LRTV and outperforms baselines. The amount of TV regularisation used in LRTV to remove aliasing in case T=250, negatively affects separability of WM and GM, and it results in (under-estimation) bias in T2 estimations for of GM and CSF.}




%\begin{figure}[t]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%\begin{turn}{90} \quad \textbf{\MCMRF} \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1521.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1522.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1523.pdf}
%\\
%\begin{turn}{90} \qquad PVMRF \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1121.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1122.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1123.pdf}
%\\
%\begin{turn}{90} \quad\quad SPIJN \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1221.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1222.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1223.pdf}
%\\
%\begin{turn}{90} \quad BayesianMRF \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1321.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1322.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1323.pdf}
%\\
%\begin{turn}{90} \quad SG-Lasso \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1421.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1422.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_1423.pdf}
%\\
%\caption{{Estimated mixture maps and their T1/T2s for the WM, GM and CSF in-vivo brain compartments using MC-MRF baselines and \MCMRF at sequence length 1000. All methods used (a) LRTV and (b) SVD-MRF reconstructions before mixture separation. 
%}\label{fig:vivo_compareMM} }
%\end{minipage}}
%\end{figure}

%\begin{figure}[t]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%\begin{turn}{90} \qquad PVMRF \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2121.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2122.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2123.pdf}
%\\
%\begin{turn}{90} \quad\quad SPIJN \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2221.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2222.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2223.pdf}
%\\
%\begin{turn}{90} \quad BayesianMRF \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2321.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2322.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2323.pdf}
%\\
%\begin{turn}{90} \quad SG-Lasso \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2421.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2422.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2423.pdf}
%\\
%\begin{turn}{90} \quad \textbf{\MCMRF} \end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2521.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2522.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe2_baselines/im_2523.pdf}
%\\
%\caption{{The estimated T1/T2 values and the (normalised) mixture maps of the WM, GM and CSF compartments using MC-MRF baselines and \MCMRF. All methods used SVD-MRF reconstruction before mixture separation. 
%}\label{fig:vivo_compareMM2} }
%\end{minipage}}
%\end{figure}


%%====== scatterplot compare baselines (SVDMRF)=====================
%
%\begin{figure*}[ht!]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%%\begin{turn}{90} \qquad PVMRF \end{turn}
%\includegraphics[width=.19\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_211.pdf}
%\includegraphics[width=.19\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_221.pdf}
%\includegraphics[width=.19\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_231.pdf}
%\includegraphics[width=.19\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_241.pdf}
%\includegraphics[width=.19\linewidth]{../figs_gen/vivo/figs_expe2_baselines/scatter_251.pdf}
%\caption{{The T1/T2 values of the estimated compartments using (from left to right) PVMRF, SPIJN, BayesianMRF, SG-Lasso and \MCMRF algorithms prior to the thresholding postprocessing. SVD-MRF reconstruction is used for all methods. Scatter points' radii are scaled by the $\ell_2$ norms of the corresponding mixture maps. 
%}\label{fig:vivo_compareScatter2} }
%\end{minipage}}
%\end{figure*}


%========== sequence cut==========

%
%\begin{figure}[ht!]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%
%\begin{turn}{90} \, \MCMRF 750\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1511.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1512.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1513.pdf}
%\\
%\begin{turn}{90} \, \MCMRF 500\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1521.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1522.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1523.pdf}
%\\
%\begin{turn}{90} \, \MCMRF 250\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1531.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1532.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1533.pdf}
%\\
%\vspace{.3cm}
%\begin{turn}{90} \quad PVMRF 750\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1111.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1112.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1113.pdf}
%\\
%\begin{turn}{90} \quad PVMRF 500\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1121.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1122.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1123.pdf}
%\\
%
%\begin{turn}{90} \quad PVMRF 250\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1131.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1132.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1133.pdf}
%\\
%\vspace{.3cm}
%\begin{turn}{90} \quad SPIJN 750\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1211.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1212.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1213.pdf}
%\\
%\begin{turn}{90} \quad SPIJN 500\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1221.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1222.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1223.pdf}
%\\
%
%\begin{turn}{90} \quad SPIJN 250\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1231.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1232.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_1233.pdf}
%\\
%
%\caption{{The estimated T1/T2 values and the (normalised) mixture maps of the WM, GM and CSF compartments using MC-MRF baselines and \MCMRF for shorter (truncated) acquisition lengths 750, 500 and 250. All methods used LRTV reconstruction before mixture separation. 
%}\label{fig:vivo_cut_lrtv} }
%\end{minipage}}
%\end{figure}
%
%\begin{figure}[ht!]
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%
%\begin{turn}{90} \, \MCMRF 750\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2511.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2512.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2513.pdf}
%\\
%\begin{turn}{90} \, \MCMRF 500\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2521.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2522.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2523.pdf}
%\\
%\begin{turn}{90} \, \MCMRF 250\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2531.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2532.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2533.pdf}
%\\
%\vspace{.3cm}
%\begin{turn}{90} \quad PVMRF 750\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2111.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2112.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2113.pdf}
%\\
%\begin{turn}{90} \quad PVMRF 500\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2121.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2122.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2123.pdf}
%\\
%
%\begin{turn}{90} \quad PVMRF 250\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2131.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2132.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2133.pdf}
%\\
%\vspace{.3cm}
%\begin{turn}{90} \quad SPIJN 750\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2211.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2212.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2213.pdf}
%\\
%\begin{turn}{90} \quad SPIJN 500\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2221.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2222.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2223.pdf}
%\\
%
%\begin{turn}{90} \quad SPIJN 250\end{turn}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2231.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2232.pdf}
%\includegraphics[width=.3\linewidth]{../figs_gen/vivo/figs_expe3_cut/im_2233.pdf}
%\\
%
%\caption{{The estimated T1/T2 values and the (normalised) mixture maps of the WM, GM and CSF compartments using MC-MRF baselines and \MCMRF for shorter (truncated) acquisition lengths 750, 500 and 250. All methods used SVD-MRF (zero-filling) reconstruction before mixture separation. 
%}\label{fig:vivo_cut_zf} }
%\end{minipage}}
%\end{figure}
%



==> sections/supp_theory.tex <==
% !TEX root = ../offgridQMRI.tex

\newcommand{\JJ}{\mathbb{J}}
\newcommand{\HH}{\mathbb{H}}

\section{Support stability}

\paragraph{Notations}
 For $\phi:\RR^d \to \RR^T$, let $\JJ_\phi(\theta) \in \RR^{T\times d}$ denote the Jacobian of $\phi$ at $\theta$.   Given a matrix $Q\in \RR^{n\times m}$, let $\vc_{n,m}(p)\in\RR^{nm}$ be its vectorized version with columns stacked vertically, let $\rc_{n,m}$ be the inverse operation, so that $\rc_{n,m}(\vc_{n,m}(p)) = p$. Finally, we define the soft-thresholding operator by $S_\beta:\RR^v \to \RR^v$ is defined by  $$S_\beta(\xi)_i = \begin{cases} \xi_i -\beta &\xi_i >\beta,
\\ \xi_i +\beta &\xi_i<-\beta,
 \\0  & \abs{\xi_i}\leq \beta.
\end{cases}.$$
Given a matrix or a tensor, we write  $\norm{\cdot}$ without subscript to denote the operator norm with respect to the vector norm $\norm{\cdot}_2$. Given an index set $I$ and a vector $V$, we denote by $\proj_I(V)$ the restriction of $V$ to the index set $I$. Given a point $x\in \RR^n$ and $r>0$, we denote by $\Bb(x,r) \eqdef \enscond{z}{\norm{x-z}<r}$ the open ball of radius $r$ around $x$.

\subsection{The precertificate as a least squares solution}\label{supp:precertificate_lsq}
We detail here how to write the solution of $Q_\btheta$ as the solution of a linear system. Observe that the constraints $\proj_{I_s}f(\theta_s) = \frac{\proj_{I_s}C_s}{\norm{C_s}_2}$ for all $s\in [k]$ can be written as
\begin{align*}
\proj_{\bold{I}} \vc_{k,v} \pa{ \Phi^\top_{\btheta} Q}= \proj_{\bold{I}} [\Id_v \otimes D_{\btheta}^\top]\vc_{T,v}(P) = u_0
\end{align*}
where $u_0 = \pa{(1-\beta) +\beta  \sqrt{v}\proj_{I_s}  C_s/\norm{C_s}_2}_{s=1}^k \in \RR^{\sum_s \abs{I_s}}$ and 
$\proj_{\bold{I}}: \RR^{kv} \to \RR^{\sum_s \abs{I_s}}$ is the  subsampling operator given  by which selects the nonzero entries of $\ens{I_s}_{s\in[k]}$, so that given a matrix $z \in \RR^{k\times v}$ with $s^{th}$ row $z_s \in \RR^{v}$ for $s\in [k]$, $\proj_{\bold{I}} \vc(z) = \pa{(z_s)_{I_s}}_{s\in [k]}$.

The constraints $\partial_\theta \norm{f(\theta_s)}_2^2 = 0$  for all $s\in [k]$ can be written as
\begin{align*}
\mathbf{0}_d &= \beta \sqrt{v} \sum_{i\in I_s}  f_i(\theta_s) \nabla f_i(\theta_s)  = \frac{1}{\norm{C_s}_2} \sum_{i=1}^v (C_s)_i \nabla [\Phi^* Q](\theta_s) \\
&= \JJ_\phi(\theta_s)^\top Q \frac{C_s}{\norm{C_s}_2} =\frac{1}{\norm{C_s}_2}[ C_s^\top\otimes \JJ_\phi(\theta_s)^\top]\vc_{T,v}(P)
\end{align*}

We can therefore define the $Tv\times (\sum_{s=1}^k \abs{I_s}+kd)$ matrix \begin{equation}\label{eq:Gamma}
\Gamma = \left[(\Id_v\otimes D_\btheta ) \proj_{\bold{I}}^* ,\frac{ C_1}{\norm{C_1}_2} \otimes \JJ_\phi(\theta_1), \cdots, ,\frac{ C_k}{\norm{C_k}_2} \otimes \JJ_\phi(\theta_k) \right]
 \end{equation}
 and write
 $$Q_\btheta = \rc_{T,v} \pa{(\Gamma^*)^\dagger \begin{pmatrix}
u_0\\
\mathbf{0}_{kd}
\end{pmatrix}}.$$ Note that $\Gamma$ depends on $\btheta$ and $\ens{C_s/\norm{C_s}_2}_s$. To make this dependence clear, we will sometimes write $\Gamma_{\btheta,C}$ in place of $\Gamma$.

\subsection{The dual of sparse group Blasso}

The proof of Theorem \ref{thm:stability} is via analysis of the dual problem to \eqref{eq:spglasso}.  The proof follows closely the proof of support stability from \cite{duval2015exact}, however, we present the details here since the case of vector-valued measured with the sparse group norm has not be covered in the literature. 
We describe the some primal dual relationships in this section.

To simplify notation, throughout this section and the next, we let  $\lambda_1 \eqdef \beta$ and $\lambda_2 \eqdef \sqrt{v}(1-\beta)$.



\paragraph{Duality for sparse group lasso}
Before describing the dual problem, we first mention a duality, described in~\footnote{O.~Burdakov and B.~Merkulov, ``On a new norm for data fitting and optimization
  problems,'' \emph{Link{\"o}ping University, Tech. Rep.
  LiTH-MAT}, 2001.}, % \cite{burdakov2001new}, 
  between the vector norm (for $x\in\RR^n$ and $\epsilon>0$), $J(x) \eqdef  \epsilon \norm{x}_1 + (1-\epsilon)\norm{x}_2$, and the so-called $\epsilon$-norm, which is defined for $\xi\in\RR^n$ as  $\nu = \norm{\xi}_\epsilon$  is the unique $\nu>0$ such that
$$
\sum_i (\abs{\xi_i} - (1-\epsilon)\nu)_+^2 - (\epsilon \nu)^2 = 0.
$$
It is shown in~\footnote{E.~Ndiaye, O.~Fercoq, A.~Gramfort, and J.~Salmon, ``Gap safe screening rules
  for sparse-group lasso,'' in \emph{Advances in neural information processing
  systems}, 2016, pp. 388--396.} Appendix E, Lemmas 1 and 2 (see also~$^4$) that \footnote{which of course can be written as: for all $\lambda_1,\lambda_2>0$, \begin{equation*}
\begin{split}
&\enscond{x+y}{\norm{x}_2 \leq \lambda_1 \nu, \norm{y}_\infty \leq\lambda_2 \nu} = \enscond{\xi}{  \norm{S_{\lambda_2}(\xi)}^2_2 \leq  (\lambda_1 \nu)^2 }
\end{split}
\end{equation*}}
\begin{equation}\label{eq:epsnorm1}
\begin{split}
&\enscond{x+y}{x,y\in\RR^d, \norm{x}_2 \leq \epsilon \nu, \norm{y}_\infty \leq (1-\epsilon) \nu} \\
&= \enscond{\xi\in \RR^d}{\norm{\xi}_\epsilon \leq \nu}
\end{split}
\end{equation}
and hence, the dual norm of $J$ is the $\epsilon$-norm. Moreover, we have the \emph{unique} $\epsilon$-decomposition
$$
\xi = S_\epsilon(\xi) + (\xi - S_\epsilon(\xi) )
$$
with $\norm{S_\epsilon(\xi)}_2 = (1-\epsilon) \norm{\xi}_\epsilon$ and $\norm{\xi - S_\epsilon(\xi) }_\infty = \epsilon\norm{\xi}_\epsilon$,
where we recall that $S_\epsilon$ is the soft-thresholding operator.

 
 \paragraph{The dual of sparse group Blasso}
 \begin{lem}\label{lem:pd}
 The dual problem to \eqref{eq:spglasso} is
 \eql{\label{eq:spglassodual}
\sup_{Q \in K} \dotp{X}{Q}_F - \alpha \norm{Q}_F^2 \tag{$\Dd_\al(X)$}
}
where $\Kk \subseteq \RR^{T\times v}$ is defined as
$$
\Kk  \eqdef 
\enscond{Q}{\eta \eqdef \Phi^* Q, \; \sum_{i=1}^v ({\eta_i(\theta)} - \lambda_1 )_+^2 \leq \lambda_2^2}
 $$
 The primal and dual problems are related by $\meas$ solves \eqref{eq:spglasso} if and only if $Q= \frac{X-\Phi \meas }{\alpha}$ solves \eqref{eq:spglassodual}.  Moreover, $\Phi^* Q \in \partial \norm{\meas}_\beta$.
 \end{lem}
\begin{proof}
By considering the dual norms of $\abs{\meas}_1$ and $\abs{\meas}_2$, it holds
\begin{equation}\label{eq:eps_decomp}
\begin{split}
&\norm{\meas}_\beta =  \sup_{\sup_\theta\norm{f(\theta)}_\infty \leq \beta} \dotp{f}{\meas} +  \sup_{\sup_\theta\norm{g(\theta)}_2  \leq \la_2} \dotp{g}{\meas}\\
&= \sup \enscond{ \dotp{f+g}{\meas} }{ \forall \theta, \; \norm{f(\theta)}_\infty \leq \la_1, \norm{g(\theta)}_2 \leq \la_2}
\end{split}
\end{equation}



%It is known from \cite{} that  for $\epsilon>0$,
%\begin{align*}
%&\enscond{x+y}{x,y\in\RR^d, \norm{x}_2 \leq \epsilon \nu, \norm{y}_\infty \leq (1-\epsilon) \nu} \\
%&= \enscond{\xi\in \RR^d}{\norm{\xi}_\epsilon \leq \nu}
%\end{align*}
%where the so-called $\epsilon$-norm, defined as $\nu = \norm{\xi}_\epsilon$  is the unique $\nu>0$ such that
%$$
%\sum_i (\abs{\xi_i} - (1-\epsilon)\nu)_+^2 - (\epsilon \nu)^2 = 0.
%$$
%Therefore,
From \eqref{eq:epsnorm1}, 
\begin{align*}
&\enscond{x+y\in\RR^d}{ \norm{x}_2 \leq \la_2 , \norm{y}_\infty \leq  \la_1 } \\
&= \enscond{\xi\in \RR^d}{ \norm{S_{\la_1}(\xi)}_2^2 \leq \la_2 }
\end{align*}
and
$
\norm{\meas}_{\beta} = 
\sup_{f\in\Kk_0}{\dotp{f}{\meas}}
$
where $$\Kk_0 = \enscond{ f\in \Cc(\Tspace;\RR^v)}{  \sup_{\theta\in\Tspace}   \norm{S_{\la_1}( f(\theta))}_2^2 \leq \la_2^2}.
$$
Note that we can restrict the set $\Kk_0$ to positive functions $\Kk_+ \eqdef \Kk_0 \cap \Cc(\Tspace;\RR_+^v)$ since $\meas$ is a positive measure.
Therefore, the convex conjugate of $J(\meas) \eqdef \norm{\meas}_\beta$ is $\iota_{\Kk_+}$, the indicator function on the set $\Kk_+$.

The result now follows by applying the Fenchel-Rockafellar duality Theorem 4.2\footnote{I.~Ekeland and R.~Temam, \emph{Convex analysis and variational problems}.\hskip
  1em plus 0.5em minus 0.4em\relax SIAM, 1999.}.  %\cite[Thm 4.2]{ekeland1999convex}.

\end{proof}

Given a dual solution $Q_\alpha$ to \eqref{eq:spglassodual}, the function  $f(\theta) \eqdef \frac{1}{\la_2  }  (\eta(\theta) - \la_1)_+$ with $\eta \eqdef \Phi^* Q_\alpha$ characterizes the support of any primal solution $\meas_\alpha$ of \eqref{eq:spglasso} in the following sense:

\begin{lem}\label{lem:structure}
Any solution $\meas_\alpha$ to \eqref{eq:spglassodual} satisfies
$$
\Supp(\meas_\alpha) \subseteq \enscond{\theta\in\Tspace}{ \norm{f(\theta)} = 1  }.
$$
 If  $\meas_\alpha = \sum_s C_s^\top \delta(\theta - \theta_s)$ is a discrete measure, then for each $s$, $\Supp(C_s) \subseteq \enscond{j \in [v]}{\eta_j(\theta_s) > \la_1}$ and $f(\theta_s) = C_s/\norm{C_s}_2$.
 
 \end{lem}
\begin{proof}

We know $\eta = \Phi^* p \in \partial \abs{\meas}_\beta = \la_1 \partial \abs{\meas}_1  + \la_2 \abs{\meas}_2$.
From
\eqref{eq:eps_decomp}, if $\xi$ satisfies $\sum_i ( \xi - \la_1)_+^2 \leq \la_2^2$
then $\norm{S_{\la_1}(\xi)}_2 \leq \la_2$ and  $\norm{\xi - S_{\la_1}(\xi)}_\infty \leq \la_1$. So $S_{\la_1}(\eta) \in \la_2 \partial \abs{\meas}_2$ which gives the first inclusion. For the second,
$$
\eta - S_{\la_1} (\eta) \in \la_1 \partial \abs{\meas}_1
$$
which means that given $s\in [k]$ and $I_s = \Supp(C_s)$,
$$
\proj_{I_s } \pa{\eta(\theta_s) - \max(\eta(\theta_s) - \la_1 ,0) } = \la_1 \proj_{I_s} \sign(C_s)
$$
If  $ \eta(\theta_s)_j < \la_1 $ for $j\in I_s$, then this equation implies that $\eta(\theta_s)_j = \la_1 \sign(C_s)_j$ which is a contradiction. Therefore, $I_s \subset \enscond{j}{\eta_j(\theta_s)>\la_1}$.


\end{proof}



Note that \eqref{eq:spglassodual} has a unique solution, since it can be seen as the projection of $X/\alpha$ onto the closed convex set $K$.  Moreover, the previous lemma shows that its solution characterises the support of any primal solution $\meas$ of \eqref{eq:spglasso}. Therefore, to understand the structure of solutions to \eqref{eq:spglasso} with   $X = \Phi \meas + w$ with $\norm{w}\leq \epsilon$, it suffices to study the solution of the dual problem \eqref{eq:spglassodual}, which we denote by $Q_{\alpha,\epsilon}$.
%\begin{lem}
%Let $Q_\alpha$ solve \eqref{eq:spglassodual}. Then, letting $\eta_\alpha \eqdef \Phi^* p_\alpha$, any solution $\meas_\alpha$ to \eqref{eq:spglassodual} satisfies
%$$
%\Supp(\meas_\alpha) \subseteq \enscond{\theta\in\Tspace}{ \sum_i (\eta_i(\theta) - \beta)_+^2 =v (1-\beta)^2  }
%$$
% and if $\meas_\alpha = \sum_s C_s^\top \delta(\theta - \theta_s)$ is a discrete measure, then for each $s$, $\Supp(C_s) \subseteq \enscond{j \in [v]}{\eta_j(\theta_s) > \beta}$.
%\end{lem}
Following \cite{duval2015exact}, we can show that $Q_{\alpha,\epsilon}$ has a limit as $\epsilon/\alpha$ and $\alpha$ converge to 0:
Define the \textit{minimal norm certificate} by
\begin{equation}
\begin{split}
Q_0 \in \argmin \enscond{\norm{Q}_F}{\eta \eqdef \Phi^* Q \in \Kk, \; \dotp{\eta}{\meas} = \norm{\meas}_\beta}.
\end{split}
\end{equation}
\begin{lem}
We have $\norm{Q_{\alpha,0} - Q_0}_F \to 0$ as $\alpha\to 0$, and
$$
\norm{Q_{\alpha,\epsilon} - Q_{\alpha, 0}}_F \leq \epsilon/\alpha.
$$
\end{lem}
\begin{proof}
The proof is omitted as it is verbatim the proof of Proposition \todo{}\ref{} in \cite{duval2015exact}
\end{proof}

\begin{rem}
The minimal norm certificate $Q_0$ is  a solution to the dual problem \eqref{eq:spglassodual} with $\alpha = 0$ and $X = \Phi \meas$. Moreover, from Lemma \ref{lem:structure}, for a discrete measure $\meas = \sum_s C_s^\top \delta(\theta-\theta_s)$, we in fact have, writing $f_Q \eqdef\frac{1}{\la_2}(\Phi^* Q - \la_1)_+$,
\begin{equation}
\begin{split}
Q_0 \in \argmin \enscond{\norm{Q}_F}{  \sup_{\theta\in\Tspace} \norm{f_Q(\theta)}_2 \leq 1 \;f_Q(\theta_s) = \frac{C_s}{\norm{C_s}_2}}.
\end{split}
\end{equation}
\end{rem}

Define $\eta_0 \eqdef \Phi^* Q_0$  and $f_0 \eqdef \frac{1}{\la_2} (\eta_0 -\la_1)_+$.
We say that $Q_0$ is nondegenerate  with respect to a sparse measure $\mestar = \sum_{s=1}^k C_s \delta(\theta - \theta_s)$ 
if it satisfies 
\begin{enumerate}
\item $\norm{f_0(\theta)}_2<1$ for all $\theta\not\in \ens{\theta_i}$
\item for each $s\in [k]$, $f_0(\theta_s) =  \frac{C_s}{\norm{C_s}_2}$.
\item  letting $g(\theta) \eqdef  \norm{f_0(\theta)}_2^2$, $g''(\theta_s) \neq 0$ for all $s\in [k]$. 
%and 
%$$
%\sum_{i\in \Supp(C_s)} ({\eta_i(\theta_s)} - \beta )_+\nabla^2 \eta_i(\theta) +\nabla \eta_i(\theta_s) [\nabla \eta_i(\theta_s) ]^\top <0
%$$
\end{enumerate}

\begin{prop}\label{prop:stability}
If $Q_0$ is nondegenerate, then provided that $\epsilon/\alpha$ and $\alpha$ are sufficiently small, the solution to \eqref{eq:spglasso} is of the form $\meas_{\alpha,\epsilon} = \sum_{j=1}^k \hat C_j \delta(\theta-\hat \theta_j)$ where $\Supp(\hat C_j) \subseteq \Supp(C_j)$.
\end{prop}
\begin{proof}
From \eqref{eq:spglassodual}, we see that the dual solution to \eqref{eq:spglassodual} can be written as the projection of $X/\alpha$ onto the set $\Kk$. 
So, from $\norm{Q_{\alpha,\epsilon}-Q_{\alpha,0}} \leq  \norm{\proj_\Kk(X/\alpha) - \proj_\Kk((X+w)/\alpha)}  \leq \norm{w}_F/\alpha$, we have that $\eta_{\al,\epsilon} \eqdef \Phi^* Q_{\al,\epsilon} \to \eta_0$ in the uniform norm as $\alpha$ and $\epsilon/\alpha$ converge to 0. So, if $\eta_0$ is non-degenerate, then given any $r>0$, provided that $\norm{w}_F/\alpha$ and $\alpha$ are sufficiently small, letting $g(\theta) \eqdef \frac{1}{\la_2^2} \norm{(\eta_{\al,\epsilon}(\theta) - \la_1)_+}^2 $, we have $g(\theta)<1$ for all $\theta \not\in  \cup_j \Bb(\theta_j,r)$, and for all $\theta\in \Bb(\theta_j,r)$, $g''(\theta) \neq 0$. So, there are at most $k$ points for which $g(\theta) = 1$.  So, by Lemma \ref{lem:structure}, given data $X =\Phi \meas + w$, we recover at most $k$ components with $\meas_{\alpha,\epsilon} = \sum_{j=1}^k \hat C_j \delta(\theta-\hat \theta_j)$. Finally, uniform convergence of $\eta_{\alpha,\epsilon}$  to $\eta_0$ also ensures that $\Supp(\hat C_j) \subseteq \Supp(C_j)$ for $\alpha$ and $\epsilon/\alpha$ sufficiently small.
\end{proof}


To establish support stability, it suffices to show that $Q_0$ is nondegenerate. 
In general, $Q_0$ does not have a closed form expression and can be hard to compute, and in practice, one computes the precertificate $Q_V$ instead: Notice that
since $\norm{f_0(\theta)}^2 \leq 1$ for all $\theta$ and $\norm{f_0(\theta_s)}_2 = 1$, it is necessary that $\partial_\theta \norm{f_0(\theta_s)}_2^2 = 0$  for all $s\in [k]$. Hence, if we add the constraint that $\sup_\theta \norm{ f_p(\theta)}\leq 1$ to the constraint set in the definition of the vanishing derivatives precertificate $\eta_V$, then we have $\eta_V = \eta_0$. In other words, if  $\sup_\theta \norm{ f_V(\theta)}\leq 1$, then we must have $\eta_V = \eta_0$, and moreover, nondegeneracy of $\eta_V$ implies  that $\eta_0 = \eta_V$ is also nondegenerate.




%We look at the following proxy of $Q_0$ which has a closed form expression: Let  $s\in [k]$ and $I_s \eqdef \Supp(C_s)$. First note that the constraint $f_0(\theta_s) = \frac{C_s}{\norm{C_s}_2}$ can be written as
%\begin{align*}
%\proj_{\bold{I}} \vc\pa{ \Phi^\top_{\btheta} Q_0}= \proj_{\bold{I}} [\Id_v \otimes D_{\btheta}^\top]\vc(Q_0) = u_0
%\end{align*}
%where $u_0 = \pa{\beta + \sqrt{v}(1-\beta) \proj_{I_s}  C_s/\norm{C_s}_2}_{s=1}^k \in \RR^{\sum_s \abs{I_s}}$ and given $Z=(Z_s)_{s=1}^k \in \RR^{k v}$, $\proj_{\bold{I}}(Z) =( \proj_{I_s} Z_s)_{s=1}^k$. Since $\norm{f_0(\theta)}^2 \leq 1$ for all $\theta$ and $\norm{f_0(\theta_s)}_2 = 1$, it is necessary that $\partial_\theta \norm{f_0(\theta_s)}_2^2 = 0$  for all $s\in [k]$, and hence,
%\begin{align*}
%\mathbf{0}_d &= \sum_{i=1}^v (C_s)_i \nabla (\eta_0)_i(\theta_s) \\
%&= \JJ_\phi(\theta_s)^\top Q_0 C_s =[ C_s^\top\otimes \JJ_\phi(\theta_s)^\top]\vc(Q_0)
%\end{align*}
%Defining the $Tv\times (\sum_{s=1}^k \abs{I_s}+kd)$ matrix $$
%\Gamma = \left[(\Id_v\otimes D_\btheta ) \proj_{\bold{I}}^* , C_1\otimes \JJ_\phi(\theta_1), \cdots, C_k \otimes \JJ_\phi(\theta_k) \right]
% $$
%we see that $Q_0$ must satisfy
%$$
%\Gamma^{*} Q_0 = \begin{pmatrix}
%u_0\\
%\mathbf{0}_{kd}
%\end{pmatrix}.
%$$
%So, if $\eta_V \eqdef \Phi^* \rc \pa{(\Gamma^*)^\dagger \begin{pmatrix}
%u_0\\
%\mathbf{0}_{kd}
%\end{pmatrix}}$ satisfies $\norm{S_\beta(\eta_V(\theta))}_2 \leq \sqrt{v}(1-\beta)$ for all $\theta$, then $\eta_V = \eta_0$ and we have a closed form expression for $\eta_0$.  

%Define $f_V(\theta)  \eqdef \frac{1}{\sqrt{v}(1-\beta)}(\eta_V(\theta) - \beta)_+$. Note that by definition, $f_V(\theta_s) = f_0(\theta_s)$. 
%\begin{defn}
%We call  $\eta_V$ the vanishing derivatives precertificate and say that it is nondegenerate if $f_V(\theta) <1$ for all $\theta \not\in \ens{\theta_s}_{s=1}^k$ and $ g_V(\theta) \eqdef  \norm{f_V(\theta)}^2$ satisfies $g_V''(\theta_s) \neq 0$ for all $s\in [k]$.
%
%\end{defn}
%Clearly, if $\eta_V$ is nondegenerate, then $\eta_V = \eta_0$ is also nondegenerate.
\subsection{A quantitative result on support stability}\label{supp:theory_proof}



To prove Theorem \ref{thm:stability}, we rely on the implicit function theorem. The classical implicit function theorem is as follows:
\begin{prop}[Implicit function theorem]\label{prop:IFT}
Let $u_0\in\RR^m$, $v_0\in \RR^n$.
Let $f: \RR^{m} \times \RR^{n}\to \RR^n$ be such that $f(u_0, v_0) = 0$ and $\partial_u f(u_0,v_0)$ is invertible. Then, there exists a neighbourhood $V$ of $v_0$ and a neighbourhood $U$ of $u_0$, and a continuously differentiable function $g:V\to U$ such that 
$$
f(u,v) = 0 \iff u = g(v).
$$
Moreover, for all $v\in V$, the Jacobian of $g$ is $$J_g(v)  =\pa{ \partial_u f(g(v), v)}^{-1} \partial_v f(g(v), v).$$


\end{prop}

Typical quantitative versions of the implicit function theorem require showing invertibility  of $\partial_u f(u,v)$  and obtaining norm bounds on the partial derivatives of $f$  in some neighbourhood of $U$ of $u_0$ and $V$ of $v_0$. A quantitative version is proved in \cite[Section 4.3]{}, which requires to look at $\partial_u f(u,v)$  only when $f(u,v) = 0$. We present their arguments below and restate their result in greater generality.  
\begin{prop} \label{prop:IFT_quant}
Let $U_0$ be an open neighbourhood of $u_0$.
Let $R_2>0$. Assume that for all $u\in U_0$ and $v\in \Bb(v_0,R)$, $f(u,v) = 0$ implies that $\partial_u f(u,v)$ is invertible and  $\norm{\partial_u f(u,v)^{-1} \partial_v f(u,v)} \leq M$. Let $r_0 \eqdef \min\enscond{\norm{u-u_0}}{u\in \partial U_0}$.

Then,  the conclusions of Proposition \ref{prop:IFT} hold with $V \supset \Bb(v_0, \min\pa{r_0/M, R})$ and $\norm{J_g(v)} \leq M$.

\end{prop}
\begin{proof}
Define $V^* \eqdef \bigcup_{V\in\Vv} V$ where $\Vv$ is the collection of all open sets such that
\begin{itemize}
\item[(i)] $v_0\in V$
\item[(ii)]  $V$ is star-shaped with respect to $v_0$,
\item[(iii)]  $V\subset \Bb(v_0, R)$
\item[(iv)]  there exists a $\Cc^1$ function $g: V \to \RR^{m}$ such that $g(v_0) = u_0$ and for all $v\in V$, $f(g(v), v) = 0$.
\item[(v)]  $g(v) \subset U_0$.
\end{itemize}
Note that $\Vv$ is non-empty since we can apply the implicit function theorem to $f$ at $u_0$, $v_0$ to obtain a set $V$ and function $g$ which satisfies (i) to (v).
The collection $\Vv$ is stable by union and we can define $g^*$ on $V^*$ by
$$
g^*(v) = g(v), \qquad \text{if} \quad v\in V, \; V\in \Vv, \; g \text{ is the corresponding function}.
$$
We simply need to show that $V^* \supset \Bb(v_0, r_0/M)$.


Let $v\in V$ be of norm 1, and define
$$
r \eqdef \sup\enscond{r>0}{ v_0+ rv \in V^*}.
$$
Then, $r\in (0, R]$. Assume that $r<R$.
Let  $v_r \eqdef v_0+r v \in V^*$ and we can define $g^*(v_r) = \lim_{r'\to r} g^*(v_0+ r'v)$.  Since $ g^*(v_0+ r'v) \in U_0$ for all $r'<r$, we have $u\in \overline{U_0}$.  We claim that $u\in \partial U_0$ is on the boundary. Suppose $u \in U_0$. Then, by assumption, $ f(g^*(v_r), v_r) = 0$ and $\partial_u f(g^*(v_r), v_r)$ is invertible, we can therefore apply the IFT to construct neighbourhoods $U'$ around $g^*(v_r)$, $V'$ around $v_r$ to define a $\Cc^1$ function $g: V' \to \RR^m$ such that $g(v_r) = g^*(v_r)$ and for all $v\in V'$, $f(g(v), v) = 0$.  We can therefore extend the set $V^*$ to a set $V_r$ such that $V^* \subsetneq V_r$. This is a contradiction to the maximality of $V^*$. So, $g^*(v_r)\in \partial U_0$. Note that for all $t\in [0,1)$,  $v_0 + t rv \in V^* \subset \Bb(v_0, R)$, so $g(v_0 + t rv) \in U_0$. So, by assumption $\norm{J_g(v_0 + tr v)} \leq M$. Therefore,
$$
r_0 \leq \norm{g^*(v_r) - u_0} =\norm{ \int_0^1 J_g(v_0 + tr v) (r v) \mathrm{d}t } \leq M r
$$
Therefore, $r\geq \frac{r_0}{M}$.

\end{proof}



\begin{thm}\label{thm:stability}
Let $\epsilon>0$ and $X = \Phi \mestar + W$ where $W \in \RR^{T\times v}$ satisfies $\norm{W}_F \leq \epsilon$ and $\mestar = \sum_{s=1}^k C^*_s \delta(\theta-\theta^*_s)$. Suppose that $\Gamma\eqdef \Gamma_{\btheta^*, C^*}$ is full rank and $\eta_V$ is nondegenerate with respect to $\mestar$, then  there exists constants $\rho_1,\rho_2,\rho_3>0$ which depend only on $\eta_V$ and $\Gamma$ such that   for all  $\epsilon/\alpha \leq \rho_1$ and
$\alpha  \leq \rho_2 \min_s \norm{C_s^*}^2 $, 
  \eqref{eq:spglasso} recovers a unique solution of the form $ \sum_{s=1}^k  C_s \delta(\theta-\theta_s)$ with 
\begin{equation}\label{eq:error_bd}
\norm{ C^* - C}_F + \norm{ \btheta^* - \btheta}_F   \leq \rho_3 \pa{ \frac{ { \epsilon+\alpha}}{\min_s \norm{C_s^*}} }
\end{equation}  

\end{thm}


\begin{proof}

The goal is to define a $\Cc^1$ function $G: \RR^{T\times v}\times \RR_+ \to \RR^{N+kd}$ such that $(C, \btheta) \eqdef G(W, \alpha)$ corresponds to  a solution of \eqref{eq:spglasso} with data $X= D_{\btheta^*} (C^*)^\top + W$. We first use the implicit function theorem to define such a $G$, then show that it does indeed define a solution to \eqref{eq:spglasso}.


To this end,  let $N= \sum_{s}\abs{I_s}$ and define a function
$$
F:\RR_+^{N} \times \Tspace^k \times \RR^{T \times v}\times  \RR_+ \to \RR^{N + kd}
$$
so that given $C = \ens{C_s}_{s\in [k]}$ with $C_s \in \RR^{\abs{I_s}}$, $\btheta\in\Tspace^k$, $W\in \RR^{T\times v}$ and $\alpha \in \RR_+$,
 $$F(C,\btheta,W,\alpha) = \begin{bmatrix}
\pa{g_s(C,\btheta,W,\alpha)}_{s=1}^k\\
\pa{h_s(C,\btheta,W,\alpha)}_{s=1}^k
\end{bmatrix}$$
where $g_s(C,\btheta,W,\alpha) \in \RR^{\abs{I_s}}$ and $h_s (C,\btheta,W,\alpha)\in \RR^{d}$ are given by
$$
g_s (C,\btheta,W,\alpha)^\top = 
\pa{ \phi(\theta_s)^\top[D_\btheta \bar C^\top -D_{\btheta^*} (C^*)^\top - W ] }_{I_s}+ \alpha \pa{ \lambda_1 +  \lambda_2 \frac{C_s^\top}{\norm{C_s}}}
$$
and
$$
h_s (C,\btheta,W,\alpha) = J_{\phi}(\theta_s)^\top \pa{D_\btheta \bar C^\top - D_{\btheta^*} (C^*)^\top- W} \frac{\bar C_s}{\norm{C_s}_2}.
$$
Here, $\bar C\in \RR^{ v\times k}$ is the matrix with $s^{th}$ column satisfying  $(\bar C_s)_{I_s} = C_s$ and $(\bar C_s)_{I_s^c} = 0$.
Clearly, if $(C,\btheta)$ correspond to a solution of \eqref{eq:spglasso} with data $X= D_{\btheta^*} (C^*)^\top + W$, then $F(C,\btheta,W,\alpha) = 0$. Note also that $F(C^*, \btheta^*, 0,0) = 0$.




The partial derivatives of $g \eqdef (g_s)$ and $h \eqdef (h_s)$ are as follows: Define \begin{equation}\label{eq:Z}
Z \eqdef D_{\btheta}\bar C^\top - D_{\btheta^*} (C^*)^\top - W,
\end{equation}
then
\begin{align*}
\partial_c g &=  \proj_{\bold{I}} \pa{\Id_{v}\otimes  \Phi^\top_{\btheta} D_{\btheta}} \proj_{\bold{I}}^* + \alpha \lambda_2 \diag \pa{\frac{1}{\norm{C_s}}\Id_{\abs{I_s}} -\frac{ C_s C_s^\top}{\norm{C_s}^3}}_{s\in[k]}
\\
\partial_\theta g &=  \diag([ Z_{(:, I_s)}]^\top \JJ_\phi(\theta_s))_{s\in[k]} + {\pa{ C_j  \phi(\theta_s)^\top \JJ_\phi(\theta_j)}}_{s,j\in [k]}  
\\
\partial_\al g &=   \pa{\lambda_1 + \lambda_2 \frac{C_s}{\norm{C_s}}}_{s\in[k]} \\
\partial_w g &= \proj_{\bold{I}} (\Id_v \otimes \Phi^\top_{\btheta})
\end{align*}


Let  $\HH_\phi(\theta)^\top \in\RR^{d\times d\times T}$ so that is $(i,j,n)$ entries with $i,j\in [d]$ for the Hessian of $\phi_n(\theta_s)$. So, given a vector  $z\eqdef (z_n)_{n=1}^T$, $\HH_\phi(\theta)^\top  z= \sum_{n=1}^T z_n \nabla^2 \phi_j(\theta) \in \RR^{d\times d}$. Then,
\begin{align*}
\partial_c h &= \diag\pa{\JJ_\phi(\theta_s)^\top Z_{(:, I_s)}  \pa{\frac{1}{\norm{C_s}_2}\Id_{\abs{I_s}} - \frac{C_s C_s^\top}{\norm{C_s}^3}   }   }_{s\in[k]} + \pa{  [\frac{1}{\norm{C_s}_2}C_s^\top \otimes \JJ_\phi(\theta)^\top] [\Id_v \otimes D_{\btheta}]}_{s\in[k]}\\
\partial_{\btheta} h &= \diag\pa{\HH_\phi(\theta_s)^\top Z \frac{\bar C_s}{\norm{C_s}_2} }_s + \pa{  \frac{1}{\norm{C_j}_2}\JJ_\phi(\theta_j)^\top \JJ_\phi(\theta_s) \bar C_j^\top \bar C_s }_{j,s\in [k]}
\\
\partial_\alpha h &= \mathbf{0}_{kd}\\
\partial_w h &= -\pa{\frac{1}{\norm{C_s}_2}C_s^\top\otimes  \JJ_\phi(\theta_s)^\top }_{s\in [k]}
\end{align*}

We therefore have
$$
\partial_{(C,\btheta)}F =\pa{ \Gamma_{\btheta,C}^\top\Gamma_{\btheta,C} +Y } \begin{pmatrix}
\Id_{N} & \mathbf{0}_{N \times kd}\\
\mathbf{0}_{kd\times N } &\diag\pa{\norm{C_s}_2}_{s=1}^k \otimes \Id_{d}
\end{pmatrix}
$$
where 
$$
Y\eqdef  \begin{pmatrix}
\alpha \lambda_2 \diag \pa{\frac{1}{\norm{C_s}}\Id_{\abs{I_s}} -\frac{ C_s C_s^\top}{\norm{C_s}^3}} & \diag\pa{\frac{1}{\norm{C_s}_2} \JJ_\phi(\theta_s)^\top Z_{(:,I_s)}   }_{s\in[k]}^\top \\
 \diag\pa{\JJ_\phi(\theta_s)^\top Z_{(:,I_s)}  \frac{1}{\norm{C_s}_2} \pa{\Id_{\abs{I_s}} - \frac{C_s C_s^\top}{\norm{C_s}_2^2}  } }_{s\in[k]} &  \diag\pa{\HH_\phi(\theta_s)^\top Z \frac{C_s}{\norm{C_s}_2^2} }_s 
\end{pmatrix},
$$
and
$$
\partial_{(\alpha,W)} F =\begin{bmatrix}
 \begin{pmatrix}
 \pa{\lambda_1 + \lambda_2 \frac{C_s}{\norm{C_s}^2}}_s\\
 \mathbf{0}_{kd}
\end{pmatrix}, &
\Gamma_{\btheta,C}^\top
\end{bmatrix}
$$

 
\textbf{Application of implicit function theorem to obtain a candidate solution.}

To apply the quantitative implicit function theorem, we first bound $\norm{\Gamma_{\btheta,C}}$ and $\norm{Y}$: Define $$S = \ens{S_s}_{s=1}^k \qandq S^* = \ens{S^*_s}_{s=1}^k \qwhereq S_s \eqdef C_s/\norm{C_s}_2 \qandq  S_s^* \eqdef C_s^*/\norm{C_s^*}_2$$
\begin{itemize} 
\item[i)] \textbf{Bound on $ \norm{\partial_{\al,W} F}$:} 

Note that by Taylor's theorem, $ \norm{D_\btheta - D_{\btheta^*}} \leq  \norm{\btheta -\btheta^*}_F \max_\theta \norm{\JJ_\phi(\btheta)}$ and
\begin{align*}
 &\norm{S_s \otimes \JJ_\phi(\theta_s) -S_s^* \otimes \JJ_\phi(\theta_s^*)} \leq
  \norm{\pa{S_s - S_s^*} \otimes \JJ_\phi(\theta_s) } + \norm{ S_s^* \otimes (\JJ_\phi(\theta_s^*) -\JJ_\phi(\theta_s)) }\\
  &\leq   \norm{S_s -S_s^* }_2 \max_\theta \norm{\JJ_\phi(\theta)} + \norm{\theta_s -\theta_s^*} \norm{S_s^*}_2 \max_\theta \norm{\HH_\phi(\theta)}.
\end{align*}
Therefore
\begin{align*}
\norm{\Gamma_{\btheta,C} - \Gamma_{\btheta^*,C^*}}^2 &\leq  \norm{D_\btheta - D_{\btheta^*}}^2 + \sum_s \norm{S_s \otimes \JJ_\phi(\theta_s) - S_s^* \otimes \JJ_\phi(\theta_s^*)}^2\\
&\leq   \norm{\btheta -\btheta^*}_F^2 \max_\theta \norm{\JJ_\phi(\btheta)}^2 +   \norm{S - S^*}_F^2 \max_\theta \norm{\JJ_\phi(\theta)}^2 + \norm{\btheta -\btheta^*}^2  \max_\theta \norm{\HH_\phi(\theta)}^2\\
&\leq  A_1^2 \pa{\norm{S-S^*}_F^2 + \norm{\btheta  - \btheta^*}_F^2}
\end{align*}
where $$A_1^2 \eqdef    \max_\theta \norm{\HH_\phi(\theta)}^2 + \max_\theta \norm{\JJ_\phi(\btheta)}^2. $$

We can apply the bounds in i)  to deduce that
\begin{equation}
 \norm{\partial_{\al,w} F}  \lesssim \norm{\Gamma_{\btheta^*,C^*}} +  A_1 \pa{\norm{S-S^*}_F + \norm{\btheta  - \btheta^*}_F}
\end{equation}



\item[ii)]
Bounds for $\partial_{(C,\btheta)} F$  when $F(C,\btheta, W, \alpha) = 0$.
%\textbf{Bounds for $\partial_{(C,\btheta)} F$ :}
 We first bound $\norm{Y}$:
 \begin{align*}
\norm{Y} \lesssim \max_s \ens{\frac{1}{\norm{C_s}_2}}  \cdot \max_s\ens{\alpha \lambda_2, \norm{ \JJ_\phi(\theta_s)^\top Z  }, \norm{\HH_\phi(\theta_s)^\top Z S_s}}
\end{align*}
Let $U \eqdef \begin{pmatrix}
  \pa{\lambda_1 + \lambda_2 C_s/\norm{C_s}_2}\\
 \mathbf{0}_{kd}
\end{pmatrix}$. Then,
$$
 \Gamma_{\btheta}^\top Z + \alpha U = 0.
$$
By applying $\Gamma_\btheta (\Gamma_\btheta^\top \Gamma_\btheta)^{-1}$ to both sides, we obtain
\begin{align*}
0 &= Z -  \proj_{\Rr(\Gamma_\btheta)}^\perp Z +\alpha (\Gamma_\btheta^\top)^\dagger  U\\
&=Z +  \proj_{\Rr(\Gamma_\btheta)}^\perp \Gamma_{\btheta^*} \binom{C^*}{\mathbf{0}_{kd}} + \proj_{\Rr(\Gamma_\btheta)}^\perp  W + \alpha (\Gamma_\btheta^\top)^\dagger  U
\end{align*}
Therefore,
$$
\norm{Z} \leq \norm{ \proj_{\Rr(\Gamma_\btheta)}^\perp D_{\btheta^*} \binom{C^*}{\mathbf{0}_{kd}}} + \norm{W} + \alpha \norm{ (\Gamma_\btheta^\top)^\dagger  U}
$$
Note that
\begin{align*}
&\proj_{\Rr(\Gamma_{\btheta,C})}^\perp D_{\btheta^* } C^*= \proj_{\Rr(\Gamma_{\btheta,C})}^\perp \sum_s \phi\pa{\theta^*_s} (C^*_s)^\top  \\
&= 
\proj_{\Rr(\Gamma_{\btheta,C})}^\perp \sum_s \Big( \phi\pa{\theta_s} (C^*_s)^\top + (\theta_s -\theta^*_s)  \JJ_\phi\pa{\theta_s} (C^*_s)^\top   + \Oo(\norm{\btheta - \btheta^*}^2_F)\Big)\\
&= 
\proj_{\Rr(\Gamma_{\btheta,C})}^\perp \sum_s \Big( \phi\pa{\theta_s} (C^*_s)^\top + (\theta_s - \theta^*_s )  \JJ_\phi\pa{\theta_s} C_s^\top  \\
&\qquad\qquad +\Oo(\norm{C^* - C}_F \norm{\btheta - \btheta^*}_F) + \Oo(\norm{\btheta - \btheta^*}^2_F)\Big)\\
&= \Oo(\norm{\btheta - \btheta^*}_F^2 + \norm{C^* - C}_F \norm{\btheta - \btheta^*}_F) 
\end{align*}
Moreover, $(\Gamma_\btheta^\top)^\dagger U = Q^* + \Oo(\norm{\btheta - \btheta^*}_F) + \Oo(\norm{S - S^*}_F)$ where
$$
Q^* \eqdef (\Gamma_{\btheta^*}^\top)^\dagger   \begin{pmatrix}
{\lambda_1 + \lambda_2 C_s^*/\norm{C_s^*}_2}\\
 \mathbf{0}_{kd}
\end{pmatrix}.
$$
Therefore,
$$
\norm{Z} = \Oo\pa{ \norm{\btheta - \btheta^*}_F + \norm{C^* - C}_F  + \alpha + \norm{W} }
$$
and where $c = \min_s \norm{C_s}$.
$$
\norm{Y} = \Oo\pa{ c^{-1} \cdot \pa{ \norm{\btheta - \btheta^*}_F^2 + \norm{C^* - C}_F^2  + \alpha + \lambda_2 \alpha + \norm{W}  } }
$$
To show that $\partial_{(C,\btheta)} F$ is invertible, note that given square matrices $A,E$ where $A$ is invertible,  $(A+E)$  is also invertible with $\norm{(A+E)^{-1}} \leq 2\norm{A^{-1}}$ provided that $\norm{E}  \leq \frac{1}{2\norm{A^{-1}}}$. 
We therefore require that 
$$
 \norm{\btheta - \btheta^*}_F + \norm{C^* - C}_F  + \alpha(1 + \lambda_2 ) + \norm{W}   = \Oo\pa{c\cdot  \norm{(\Gamma_{\btheta^*}^\top \Gamma_{\btheta^*})^{-1}}^{-1}}
$$
\end{itemize}

We can therefore apply Proposition \ref{prop:IFT_quant} with $u_0 = (C^*, \btheta^*)$, $v_0 = (0, \mathbf{0}_{k\times d})$, $r_0 = r^*$, $R =  \Oo\pa{\frac{c}{1+\lambda_2}\cdot  \norm{(\Gamma_{\btheta^*}^\top \Gamma_{\btheta^*})^{-1}}^{-1}}$,
$$
U_0 = \Bb(C^*, r^*)  \times \Bb(\btheta^*, r^*) 
$$
where $r^* =  \Oo\pa{c\cdot  \norm{(\Gamma_{\btheta^*}^\top \Gamma_{\btheta^*})^{-1}}^{-1}}$ and $M= \Oo\pa{ \norm{(\Gamma_{\btheta^*}^\top \Gamma_{\btheta^*})^{-1}} /c}$  We can therefore define
$$
G : \Bb(v_0, R_0) \to  \RR^{N+kd}
, \qwhereq R_0 =\Oo( c^2 \cdot  \norm{(\Gamma_{\btheta^*}^\top \Gamma_{\btheta^*})^{-1}}^{-1}  )
$$
so that $G(\alpha, W) = (C,\btheta)$ if and only if $F(C,\btheta,\alpha,W) = 0$, and
$$
\norm{C-C^*}_F+ \norm{\btheta - \btheta^*}_F \lesssim (\alpha+\norm{W}_F)/c.
$$


\textbf{Verifying the candidate solution.}
Finally, it remains to check  that $G(\alpha, W) = (C,\btheta)$ does indeed correspond to a solution: it suffices to check that $$Q \eqdef \frac{-1}{\alpha}Z = \frac{-1}{\alpha} (D_{\btheta} \bar C - D_{\btheta^*} C^* - W)$$ satisfies the primal dual relationships (see Lemma \ref{lem:pd}). In particular, we need to check that $\eta \eqdef \Phi^* P$ satisfies $ \sup_{\theta\in\Tspace} \norm{ \frac{1}{\lambda_2}(\eta(\theta) - \lambda_1)_+}_2 \leq 1$.
Note that $F(C,\btheta,\alpha,W) = 0$ can be rewritten as
$$
\Gamma_{\btheta,C}^\top Z  = -  \begin{pmatrix}
 \alpha(\lambda_1 + \lambda_2 \frac{C_s}{\norm{C_s}})_{s\in[k]}\\
 \mathbf{0}_{kd}
\end{pmatrix} .
$$
 By applying $\Gamma_{\btheta,C} (\Gamma_{\btheta,C}^\top\Gamma_{\btheta,C})^{-1}$ to this equation and recalling that $\proj_{\Rr(\Gamma_{\btheta,C})} \eqdef \Gamma_{\btheta,C} (\Gamma_{\btheta,C}^\top\Gamma_{\btheta,C})^{-1} \Gamma_{\btheta,C}^\top$ is the orthogonal projection onto the range of $\Gamma_{\btheta,C}$, we obtain
\begin{align*}
-\frac{1}{\al} Z =  (\Gamma_{\btheta,C}^\top)^\dagger u_0
-\frac{1}{\alpha} \proj_{\Rr(\Gamma_{\btheta,C})}^\perp  (D_{\btheta^*} C^* + W)
\end{align*}
It therefore follows that $Q = Q_V  -\frac{1}{\alpha} \proj_{\Rr(\Gamma_{\btheta,C})}^\perp  (D_{\btheta^*} C^* + W)$.  Let $\eta \eqdef \Phi^* P$. We need to show that $g(\theta) \eqdef \norm{\frac{1}{\lambda_2}[\eta(\theta) - \lambda_1]_+ }^2_2$ satisfies
\begin{itemize}
\item[i)] $g(\theta) <1$ for all $\theta \not\in \btheta$
\item[ii)]  $g''(\theta_s) \neq 0$ for all $s\in [k]$. 
\end{itemize}
Note that since $\abs{\eta(\theta)  - \eta_V(\theta)} \leq \max_\theta \norm{\phi(\theta)}_2 \norm{Q - Q_V}_F =  \norm{Q - Q_V}_F$
and
$$
\abs{\eta(\theta)  - \eta_V(\theta)} \leq \max_\theta \norm{\HH_\phi(\theta)} \norm{Q - Q_V}_F,
$$
 provided that $  \norm{Q - Q_V}_F$ is sufficiently small, we have $\eta_i(\theta)>\lambda_1$  whenever  $(\eta_V)_i(\theta)>\lambda_1$ and $g$ satisfies i) and ii) since $\eta_V$ is nondegenerate.

%Note that for scalars $a,b$, $$\abs{\max(a,0)^2 - \max(b,0)^2}  \leq ( \max(a,0) +  \max(b,0)) \cdot \abs{a-b} \leq \abs{a-b}^2 +2\max(b,0)\cdot \abs{a-b}$$
%so,
%\begin{align*}
%\abs{g(\theta) - g_V(\theta) } &\leq
%\frac{1}{\lambda_2} \sum_{i=1}^v \abs{[\eta_i (\theta) - \lambda_1]_+^2 - [(\eta_V)_i (\theta) - \lambda_1]_+ ^2  }\\
%&\leq \frac{1}{\lambda_2} \sum_{i=1}^v \abs{\eta_i (\theta) -(\eta_V)_i (\theta) }^2 + 2  [(\eta_V)_i (\theta) - \lambda_1]_+ \abs{\eta_i (\theta) -(\eta_V)_i (\theta) }\\
%&\leq \frac{1}{\lambda_2} \pa{ \norm{\eta(\theta) - \eta_V(\theta)}^2_2 + 2 \sqrt{g_V(\theta)} \norm{\eta(\theta) - \eta_V(\theta)}_2}\\
%&\leq \frac{1}{\lambda_2} \pa{  \norm{\phi(\theta)}_2^2 \norm{P-Q_V}^2_F + 2 \sqrt{g_V(\theta)}  \norm{\phi(\theta)}_2\norm{P-Q_V}_F}\\
%&=\frac{1}{\lambda_2} \pa{ \norm{P-Q_V}^2_F + 2 \sqrt{g_V(\theta)}  \norm{P-Q_V}_F}
%\end{align*}
%Similarly,
%$$
%\norm{\nabla^2 g(\theta) - \nabla^2 g_V(\theta)} \leq \frac{1}{\lambda_2} \pa{  \norm{\nabla^2 \phi(\theta)}_2^2 \norm{P-Q_V}^2_F + 2 \sqrt{g_V(\theta)}  \norm{\nabla^2 \phi(\theta)}_2\norm{P-Q_V}_F}
%$$



 
% and $\max_\theta \norm{\partial^{(j)} \eta(\theta) -\partial^{(j)} \eta_V(\theta)} \lesssim \norm{Q_V - Q}_F$ where the hidden constant depends only on $\max_{\theta}\norm{\partial^{(j)} \phi(\theta)}$,  
 
 It is enough to show that $\norm{Q_V - Q}_F \leq \rho$ for a sufficiently small constant $\rho$ (which depends only on $\eta_V$, and in particular, $\min_{i\in I_s} (\eta_V)_i(\theta^*_s) - \lambda_1$, $g_V''(\theta^*_s)$ and $1-g_V(\theta)$ for $\theta \not\in  \cup_s \Bb(\theta^*_s,r)$ where $r$ is such that $\min_{\theta\in \Bb(\theta_s,r)}\abs{g_V''(\theta)}\geq \frac12 \abs{g_V''(\theta_s)}$ ). Note that
\begin{align*}
&\proj_{\Rr(\Gamma_{\btheta,C})}^\perp D_{\btheta^* } C^*= \proj_{\Rr(\Gamma_{\btheta,C})}^\perp \sum_s \phi\pa{\theta^*_s} (C^*_s)^\top  \\
&= 
\proj_{\Rr(\Gamma_{\btheta,C})}^\perp \sum_s \Big( \phi\pa{\theta_s} (C^*_s)^\top + (\theta_s -( \theta_0)_s)  \JJ_\phi\pa{\theta_s} (C^*_s)^\top  \\
&\qquad\qquad + \Oo(\norm{\btheta - \btheta^*}^2_F)\Big)\\
&= 
\proj_{\Rr(\Gamma_{\btheta,C})}^\perp \sum_s \Big( \phi\pa{\theta_s} (C^*_s)^\top + (\theta_s -( \theta_0)_s)  \JJ_\phi\pa{\theta_s} C_s^\top  \\
&\qquad\qquad +\Oo(\norm{C^* - C}_F \norm{\btheta - \btheta^*}_F) + \Oo(\norm{\btheta - \btheta^*}^2_F)\Big)\\
&= \Oo(\norm{\btheta - \btheta^*}_F^2 + \norm{C^* - C}_F \norm{\btheta - \btheta^*}_F) = \Oo(\alpha^2/c^2)
\end{align*}
So, $Q = Q_V + \Oo( \norm{W}_F/\alpha + \alpha/c^2)$, and so, $C,\btheta$ define a solution provided that $\norm{W}_F/\alpha + \alpha/c^2 = \Oo(1)$.


\end{proof}





==> sections/supp_theory_old.tex <==
% !TEX root = ../offgridQMRI.tex

\newcommand{\JJ}{\mathbb{J}}
\newcommand{\HH}{\mathbb{H}}

\section{Support stability}

\paragraph{Notations}
 For $\phi:\RR^d \to \RR^T$, let $\JJ_\phi(\theta) \in \RR^{T\times d}$ denote the Jacobian of $\phi$ at $\theta$.   Given a matrix $Q\in \RR^{n\times m}$, let $\vc_{n,m}(p)\in\RR^{nm}$ be its vectorized version with columns stacked vertically, let $\rc_{n,m}$ be the inverse operation, so that $\rc_{n,m}(\vc_{n,m}(p)) = p$. Finally, we define the soft-thresholding operator by $S_\beta:\RR^v \to \RR^v$ is defined by  $$S_\beta(\xi)_i = \begin{cases} \xi_i -\beta &\xi_i >\beta,
\\ \xi_i +\beta &\xi_i<-\beta,
 \\0  & \abs{\xi_i}\leq \beta.
\end{cases}.$$
Given a matrix or a tensor, we write  $\norm{\cdot}$ without subscript to denote the operator norm with respect to the vector norm $\norm{\cdot}_2$. Given an index set $I$ and a vector $V$, we denote by $\proj_I(V)$ the restriction of $V$ to the index set $I$. Given a point $x\in \RR^n$ and $r>0$, we denote by $\Bb(x,r) \eqdef \enscond{z}{\norm{x-z}<r}$ the open ball of radius $r$ around $x$.

\subsection{The precertificate as a least squares solution}\label{supp:precertificate_lsq}
We detail here how to write the solution of $Q_V$ as the solution of a linear system. Observe that the constraints $\proj_{I_s}f(\theta_s) = \frac{\proj_{I_s}C_s}{\norm{C_s}_2}$ for all $s\in [k]$ can be written as
\begin{align*}
\proj_{\bold{I}} \vc_{k,v} \pa{ \Phi^\top_{\btheta} Q}= \proj_{\bold{I}} [\Id_v \otimes D_{\btheta}^\top]\vc_{T,v}(P) = u_0
\end{align*}
where $u_0 = \pa{(1-\beta) +\beta  \sqrt{v}\proj_{I_s}  C_s/\norm{C_s}_2}_{s=1}^k \in \RR^{\sum_s \abs{I_s}}$ and 
$\proj_{\bold{I}}: \RR^{kv} \to \RR^{\sum_s \abs{I_s}}$ is the  subsampling operator given  by which selects the nonzero entries of $\ens{I_s}_{s\in[k]}$, so that given a matrix $z \in \RR^{k\times v}$ with $s^{th}$ row $z_s \in \RR^{v}$ for $s\in [k]$, $\proj_{\bold{I}} \vc(z) = \pa{(z_s)_{I_s}}_{s\in [k]}$.

The constraints $\partial_\theta \norm{f(\theta_s)}_2^2 = 0$  for all $s\in [k]$ can be written as
\begin{align*}
\mathbf{0}_d &= \beta \sqrt{v} \sum_{i\in I_s}  f_i(\theta_s) \nabla f_i(\theta_s)  = \frac{1}{\norm{C_s}_2} \sum_{i=1}^v (C_s)_i \nabla [\Phi^* Q](\theta_s) \\
&= \JJ_\phi(\theta_s)^\top Q \frac{C_s}{\norm{C_s}_2} =\frac{1}{\norm{C_s}_2}[ C_s^\top\otimes \JJ_\phi(\theta_s)^\top]\vc_{T,v}(P)
\end{align*}

We can therefore define the $Tv\times (\sum_{s=1}^k \abs{I_s}+kd)$ matrix \begin{equation}\label{eq:Gamma}
\Gamma = \left[(\Id_v\otimes D_\btheta ) \proj_{\bold{I}}^* ,\frac{ C_1}{\norm{C_1}_2} \otimes \JJ_\phi(\theta_1), \cdots, ,\frac{ C_k}{\norm{C_k}_2} \otimes \JJ_\phi(\theta_k) \right]
 \end{equation}
 and write
 $Q_V = \rc_{T,v} \pa{(\Gamma^*)^\dagger \begin{pmatrix}
u_0\\
\mathbf{0}_{kd}
\end{pmatrix}}$. Note that $\Gamma$ depends on $\btheta$ and $C$. To make this dependence clear, we will sometimes write $\Gamma_{\btheta,C}$ in place of $\Gamma$.

\subsection{The dual of sparse group Blasso}

The proof of Theorem \ref{thm:stability} is via analysis of the dual problem to \eqref{eq:spglasso}.  The proof follows closely the proof of support stability from \cite{duval2015exact}, however, we present the details here since the case of vector-valued measured with the sparse group norm has not be covered in the literature. 
We describe the some primal dual relationships in this section.

To simplify notation, throughout this section and the next, we let  $\lambda_1 \eqdef \beta$ and $\lambda_2 \eqdef \sqrt{v}(1-\beta)$.



\paragraph{Duality for sparse group lasso}
Before describing the dual problem, we first mention a duality, described in \cite{burdakov2001new}, between the vector norm (for $x\in\RR^n$ and $\epsilon>0$), $J(x) \eqdef  \epsilon \norm{x}_1 + (1-\epsilon)\norm{x}_2$, and the so-called $\epsilon$-norm, which is defined for $\xi\in\RR^n$ as  $\nu = \norm{\xi}_\epsilon$  is the unique $\nu>0$ such that
$$
\sum_i (\abs{\xi_i} - (1-\epsilon)\nu)_+^2 - (\epsilon \nu)^2 = 0.
$$
It is shown in \cite[Appendix E, Lemmas 1 and 2]{ndiaye2016gap} (see also \cite{burdakov2001new}) that \footnote{which of course can be written as: for all $\lambda_1,\lambda_2>0$, \begin{equation*}
\begin{split}
&\enscond{x+y}{\norm{x}_2 \leq \lambda_1 \nu, \norm{y}_\infty \leq\lambda_2 \nu} = \enscond{\xi}{  \norm{S_{\lambda_2}(\xi)}^2_2 \leq  (\lambda_1 \nu)^2 }
\end{split}
\end{equation*}}
\begin{equation}\label{eq:epsnorm1}
\begin{split}
&\enscond{x+y}{x,y\in\RR^d, \norm{x}_2 \leq \epsilon \nu, \norm{y}_\infty \leq (1-\epsilon) \nu} \\
&= \enscond{\xi\in \RR^d}{\norm{\xi}_\epsilon \leq \nu}
\end{split}
\end{equation}
and hence, the dual norm of $J$ is the $\epsilon$-norm. Moreover, we have the \emph{unique} $\epsilon$-decomposition
$$
\xi = S_\epsilon(\xi) + (\xi - S_\epsilon(\xi) )
$$
with $\norm{S_\epsilon(\xi)}_2 = (1-\epsilon) \norm{\xi}_\epsilon$ and $\norm{\xi - S_\epsilon(\xi) }_\infty = \epsilon\norm{\xi}_\epsilon$,
where we recall that $S_\epsilon$ is the soft-thresholding operator.

 
 \paragraph{The dual of sparse group Blasso}
 \begin{lem}\label{lem:pd}
 The dual problem to \eqref{eq:spglasso} is
 \eql{\label{eq:spglassodual}
\sup_{Q \in K} \dotp{X}{Q}_F - \alpha \norm{Q}_F^2 \tag{$\Dd_\al(X)$}
}
where $\Kk \subseteq \RR^{T\times v}$ is defined as
$$
\Kk  \eqdef 
\enscond{Q}{\eta \eqdef \Phi^* Q, \; \sum_{i=1}^v ({\eta_i(\theta)} - \lambda_1 )_+^2 \leq \lambda_2^2}
 $$
 The primal and dual problems are related by $\meas$ solves \eqref{eq:spglasso} if and only if $Q= \frac{X-\Phi \meas }{\alpha}$ solves \eqref{eq:spglassodual}.  Moreover, $\Phi^* Q \in \partial \norm{\meas}_\beta$.
 \end{lem}
\begin{proof}
By considering the dual norms of $\abs{\meas}_1$ and $\abs{\meas}_2$, it holds
\begin{equation}\label{eq:eps_decomp}
\begin{split}
&\norm{\meas}_\beta =  \sup_{\sup_\theta\norm{f(\theta)}_\infty \leq \beta} \dotp{f}{\meas} +  \sup_{\sup_\theta\norm{g(\theta)}_2  \leq \la_2} \dotp{g}{\meas}\\
&= \sup \enscond{ \dotp{f+g}{\meas} }{ \forall \theta, \; \norm{f(\theta)}_\infty \leq \la_1, \norm{g(\theta)}_2 \leq \la_2}
\end{split}
\end{equation}



%It is known from \cite{} that  for $\epsilon>0$,
%\begin{align*}
%&\enscond{x+y}{x,y\in\RR^d, \norm{x}_2 \leq \epsilon \nu, \norm{y}_\infty \leq (1-\epsilon) \nu} \\
%&= \enscond{\xi\in \RR^d}{\norm{\xi}_\epsilon \leq \nu}
%\end{align*}
%where the so-called $\epsilon$-norm, defined as $\nu = \norm{\xi}_\epsilon$  is the unique $\nu>0$ such that
%$$
%\sum_i (\abs{\xi_i} - (1-\epsilon)\nu)_+^2 - (\epsilon \nu)^2 = 0.
%$$
%Therefore,
From \eqref{eq:epsnorm1}, 
\begin{align*}
&\enscond{x+y\in\RR^d}{ \norm{x}_2 \leq \la_2 , \norm{y}_\infty \leq  \la_1 } \\
&= \enscond{\xi\in \RR^d}{ \norm{S_{\la_1}(\xi)}_2^2 \leq \la_2 }
\end{align*}
and
$
\norm{\meas}_{\beta} = 
\sup_{f\in\Kk_0}{\dotp{f}{\meas}}
$
where $$\Kk_0 = \enscond{ f\in \Cc(\Tspace;\RR^v)}{  \sup_{\theta\in\Tspace}   \norm{S_{\la_1}( f(\theta))}_2^2 \leq \la_2^2}.
$$
Note that we can restrict the set $\Kk_0$ to positive functions $\Kk_+ \eqdef \Kk_0 \cap \Cc(\Tspace;\RR_+^v)$ since $\meas$ is a positive measure.
Therefore, the convex conjugate of $J(\meas) \eqdef \norm{\meas}_\beta$ is $\iota_{\Kk_+}$, the indicator function on the set $\Kk_+$.

The result now follows by applying the Fenchel-Rockafellar duality theorem \cite[Thm 4.2]{ekeland1999convex}.

\end{proof}

Given a dual solution $Q_\alpha$ to \eqref{eq:spglassodual}, the function  $f(\theta) \eqdef \frac{1}{\la_2  }  (\eta(\theta) - \la_1)_+$ with $\eta \eqdef \Phi^* Q_\alpha$ characterizes the support of any primal solution $\meas_\alpha$ of \eqref{eq:spglasso} in the following sense:

\begin{lem}\label{lem:structure}
Any solution $\meas_\alpha$ to \eqref{eq:spglassodual} satisfies
$$
\Supp(\meas_\alpha) \subseteq \enscond{\theta\in\Tspace}{ \norm{f(\theta)} = 1  }.
$$
 If  $\meas_\alpha = \sum_s C_s^\top \delta(\theta - \theta_s)$ is a discrete measure, then for each $s$, $\Supp(C_s) \subseteq \enscond{j \in [v]}{\eta_j(\theta_s) > \la_1}$ and $f(\theta_s) = C_s/\norm{C_s}_2$.
 
 \end{lem}
\begin{proof}

We know $\eta = \Phi^* p \in \partial \abs{\meas}_\beta = \la_1 \partial \abs{\meas}_1  + \la_2 \abs{\meas}_2$.
From
\eqref{eq:eps_decomp}, if $\xi$ satisfies $\sum_i ( \xi - \la_1)_+^2 \leq \la_2^2$
then $\norm{S_{\la_1}(\xi)}_2 \leq \la_2$ and  $\norm{\xi - S_{\la_1}(\xi)}_\infty \leq \la_1$. So $S_{\la_1}(\eta) \in \la_2 \partial \abs{\meas}_2$ which gives the first inclusion. For the second,
$$
\eta - S_{\la_1} (\eta) \in \la_1 \partial \abs{\meas}_1
$$
which means that given $s\in [k]$ and $I_s = \Supp(C_s)$,
$$
\proj_{I_s } \pa{\eta(\theta_s) - \max(\eta(\theta_s) - \la_1 ,0) } = \la_1 \proj_{I_s} \sign(C_s)
$$
If  $ \eta(\theta_s)_j < \la_1 $ for $j\in I_s$, then this equation implies that $\eta(\theta_s)_j = \la_1 \sign(C_s)_j$ which is a contradiction. Therefore, $I_s \subset \enscond{j}{\eta_j(\theta_s)>\la_1}$.


\end{proof}



Note that \eqref{eq:spglassodual} has a unique solution, since it can be seen as the projection of $X/\alpha$ onto the closed convex set $K$.  Moreover, the previous lemma shows that its solution characterises the support of any primal solution $\meas$ of \eqref{eq:spglasso}. Therefore, to understand the structure of solutions to \eqref{eq:spglasso} with   $X = \Phi \meas + w$ with $\norm{w}\leq \epsilon$, it suffices to study the solution of the dual problem \eqref{eq:spglassodual}, which we denote by $Q_{\alpha,\epsilon}$.
%\begin{lem}
%Let $Q_\alpha$ solve \eqref{eq:spglassodual}. Then, letting $\eta_\alpha \eqdef \Phi^* p_\alpha$, any solution $\meas_\alpha$ to \eqref{eq:spglassodual} satisfies
%$$
%\Supp(\meas_\alpha) \subseteq \enscond{\theta\in\Tspace}{ \sum_i (\eta_i(\theta) - \beta)_+^2 =v (1-\beta)^2  }
%$$
% and if $\meas_\alpha = \sum_s C_s^\top \delta(\theta - \theta_s)$ is a discrete measure, then for each $s$, $\Supp(C_s) \subseteq \enscond{j \in [v]}{\eta_j(\theta_s) > \beta}$.
%\end{lem}
Following \cite{duval2015exact}, we can show that $Q_{\alpha,\epsilon}$ has a limit as $\epsilon/\alpha$ and $\alpha$ converge to 0:
Define the \textit{minimal norm certificate} by
\begin{equation}
\begin{split}
Q_0 \in \argmin \enscond{\norm{Q}_F}{\eta \eqdef \Phi^* Q \in \Kk, \; \dotp{\eta}{\meas} = \norm{\meas}_\beta}.
\end{split}
\end{equation}
\begin{lem}
We have $\norm{Q_{\alpha,0} - Q_0}_F \to 0$ as $\alpha\to 0$, and
$$
\norm{Q_{\alpha,\epsilon} - Q_{\alpha, 0}}_F \leq \epsilon/\alpha.
$$
\end{lem}
\begin{proof}
The proof is omitted as it is verbatim the proof of Proposition \ref{} in \cite{duval2015exact}
\end{proof}

\begin{rem}
The minimal norm certificate $Q_0$ is  a solution to the dual problem \eqref{eq:spglassodual} with $\alpha = 0$ and $X = \Phi \meas$. Moreover, from Lemma \ref{lem:structure}, for a discrete measure $\meas = \sum_s C_s^\top \delta_{\theta_s}$, we in fact have, writing $f_Q \eqdef\frac{1}{\la_2}(\Phi^* Q - \la_1)_+$,
\begin{equation}
\begin{split}
Q_0 \in \argmin \enscond{\norm{Q}_F}{  \sup_{\theta\in\Tspace} \norm{f_Q(\theta)}_2 \leq 1 \;f_Q(\theta_s) = \frac{C_s}{\norm{C_s}_2}}.
\end{split}
\end{equation}
\end{rem}

Define $\eta_0 \eqdef \Phi^* Q_0$  and $f_0 \eqdef \frac{1}{\la_2} (\eta_0 -\la_1)_+$.
We say that $Q_0$ is nondegenerate  with respect to a sparse measure $\mestar = \sum_{s=1}^k C_s \delta(\theta - \theta_s)$ 
satisfies 
\begin{enumerate}
\item $\norm{f_0(\theta)}_2<1$ for all $\theta\not\in \ens{\theta_i}$
\item for each $s\in [k]$, $f_0(\theta_s) =  \frac{C_s}{\norm{C_s}_2}$.
\item  letting $g(\theta) \eqdef  \norm{f_0(\theta)}_2^2$, $g''(\theta_s) \neq 0$ for all $s\in [k]$. 
%and 
%$$
%\sum_{i\in \Supp(C_s)} ({\eta_i(\theta_s)} - \beta )_+\nabla^2 \eta_i(\theta) +\nabla \eta_i(\theta_s) [\nabla \eta_i(\theta_s) ]^\top <0
%$$
\end{enumerate}

\begin{prop}\label{prop:stability}
If $Q_0$ is nondegenerate, then provided that $\epsilon/\alpha$ and $\alpha$ are sufficiently small, the solution to \eqref{eq:spglasso} is of the form $\meas_{\alpha,\epsilon} = \sum_{j=1}^k \hat C_j \delta_{\hat \theta_j}$ where $\Supp(\hat C_j) \subseteq \Supp(C_j)$.
\end{prop}
\begin{proof}
From \eqref{eq:spglassodual}, we see that the dual solution to \eqref{eq:spglassodual} can be written as the projection of $X/\alpha$ onto the set $\Kk$. 
So, from $\norm{Q_{\alpha,\epsilon}-Q_{\alpha,0}} \leq  \norm{\proj_\Kk(X/\alpha) - \proj_\Kk((X+w)/\alpha)}  \leq \norm{w}_F/\alpha$, we have that $\eta_{\al,\epsilon} \eqdef \Phi^* Q_{\al,\epsilon} \to \eta_0$ in the uniform norm as $\alpha$ and $\epsilon/\alpha$ converge to 0. So, if $\eta_0$ is non-degenerate, then given any $r>0$, provided that $\norm{w}_F/\alpha$ and $\alpha$ are sufficiently small, letting $g(\theta) \eqdef \frac{1}{\la_2^2} \norm{(\eta_{\al,\epsilon}(\theta) - \la_1)_+}^2 $, we have $g(\theta)<1$ for all $\theta \not\in  \cup_j \Bb(\theta_j,r)$, and for all $\theta\in \Bb(\theta_j,r)$, $g''(\theta) \neq 0$. So, there are at most $k$ points for which $g(\theta) = 1$.  So, by Lemma \ref{lem:structure}, given data $X =\Phi \meas + w$, we recover at most $k$ components with $\meas_{\alpha,\epsilon} = \sum_{j=1}^k \hat C_j \delta_{\hat \theta_j}$. Finally, uniform convergence of $\eta_{\alpha,\epsilon}$  to $\eta_0$ also ensures that $\Supp(\hat C_j) \subseteq \Supp(C_j)$ for $\alpha$ and $\epsilon/\alpha$ sufficiently small.
\end{proof}


To establish support stability, it suffices to show that $Q_0$ is nondegenerate. 
In general, $Q_0$ does not have a closed form expression and can be hard to compute, and in practice, one computes the precertificate $Q_V$ instead: Notice that
since $\norm{f_0(\theta)}^2 \leq 1$ for all $\theta$ and $\norm{f_0(\theta_s)}_2 = 1$, it is necessary that $\partial_\theta \norm{f_0(\theta_s)}_2^2 = 0$  for all $s\in [k]$. Hence, if we add the constraint that $\sup_\theta \norm{ f_p(\theta)}\leq 1$ to the constraint set in the definition of the vanishing derivatives precertificate $\eta_V$, then we have $\eta_V = \eta_0$. In other words, if  $\sup_\theta \norm{ f_V(\theta)}\leq 1$, then we must have $\eta_V = \eta_0$, and moreover, nondegeneracy of $\eta_V$ implies  that $\eta_0 = \eta_V$ is also nondegenerate.




%We look at the following proxy of $Q_0$ which has a closed form expression: Let  $s\in [k]$ and $I_s \eqdef \Supp(C_s)$. First note that the constraint $f_0(\theta_s) = \frac{C_s}{\norm{C_s}_2}$ can be written as
%\begin{align*}
%\proj_{\bold{I}} \vc\pa{ \Phi^\top_{\btheta} Q_0}= \proj_{\bold{I}} [\Id_v \otimes D_{\btheta}^\top]\vc(Q_0) = u_0
%\end{align*}
%where $u_0 = \pa{\beta + \sqrt{v}(1-\beta) \proj_{I_s}  C_s/\norm{C_s}_2}_{s=1}^k \in \RR^{\sum_s \abs{I_s}}$ and given $Z=(Z_s)_{s=1}^k \in \RR^{k v}$, $\proj_{\bold{I}}(Z) =( \proj_{I_s} Z_s)_{s=1}^k$. Since $\norm{f_0(\theta)}^2 \leq 1$ for all $\theta$ and $\norm{f_0(\theta_s)}_2 = 1$, it is necessary that $\partial_\theta \norm{f_0(\theta_s)}_2^2 = 0$  for all $s\in [k]$, and hence,
%\begin{align*}
%\mathbf{0}_d &= \sum_{i=1}^v (C_s)_i \nabla (\eta_0)_i(\theta_s) \\
%&= \JJ_\phi(\theta_s)^\top Q_0 C_s =[ C_s^\top\otimes \JJ_\phi(\theta_s)^\top]\vc(Q_0)
%\end{align*}
%Defining the $Tv\times (\sum_{s=1}^k \abs{I_s}+kd)$ matrix $$
%\Gamma = \left[(\Id_v\otimes D_\btheta ) \proj_{\bold{I}}^* , C_1\otimes \JJ_\phi(\theta_1), \cdots, C_k \otimes \JJ_\phi(\theta_k) \right]
% $$
%we see that $Q_0$ must satisfy
%$$
%\Gamma^{*} Q_0 = \begin{pmatrix}
%u_0\\
%\mathbf{0}_{kd}
%\end{pmatrix}.
%$$
%So, if $\eta_V \eqdef \Phi^* \rc \pa{(\Gamma^*)^\dagger \begin{pmatrix}
%u_0\\
%\mathbf{0}_{kd}
%\end{pmatrix}}$ satisfies $\norm{S_\beta(\eta_V(\theta))}_2 \leq \sqrt{v}(1-\beta)$ for all $\theta$, then $\eta_V = \eta_0$ and we have a closed form expression for $\eta_0$.  

%Define $f_V(\theta)  \eqdef \frac{1}{\sqrt{v}(1-\beta)}(\eta_V(\theta) - \beta)_+$. Note that by definition, $f_V(\theta_s) = f_0(\theta_s)$. 
%\begin{defn}
%We call  $\eta_V$ the vanishing derivatives precertificate and say that it is nondegenerate if $f_V(\theta) <1$ for all $\theta \not\in \ens{\theta_s}_{s=1}^k$ and $ g_V(\theta) \eqdef  \norm{f_V(\theta)}^2$ satisfies $g_V''(\theta_s) \neq 0$ for all $s\in [k]$.
%
%\end{defn}
%Clearly, if $\eta_V$ is nondegenerate, then $\eta_V = \eta_0$ is also nondegenerate.
\subsection{Proof of Theorem \ref{thm:stability}}\label{supp:theory_proof}


%\begin{thm}\label{thm:stability}
%Let $X = \Phi \mestar + \epsilon$ where $\epsilon \in \RR^{T\times v}$ satisfies $\norm{\epsilon}_F \leq \delta$ and $\mestar = \sum_{s=1}^k C_s \delta_{\theta_s}$. Suppose that $\Gamma$ is full rank and $\eta_0 \eqdef \Phi^* Q_0$ is nondegenerate, then for all $\alpha$ and $\delta/\alpha$ sufficiently small,  \eqref{eq:spglasso} recovers a unique solution of the form $ \sum_{s=1}^k \tilde C_s \delta(\theta - \tilde \theta_s)$ with $\norm{\tilde C_s - C_s}_F \leq \delta$ and $\norm{\tilde \theta_s - \theta_s} \leq \delta$.
%
%\end{thm}





\begin{proof}[Proof of Theorem \ref{thm:stability}]


Let $\mestar =  \sum_s (C^*_s)^\top {\delta}_{\theta^*_s}$.
We already know from Proposition \ref{prop:stability} that for small $\alpha$ and $\epsilon/\alpha$, the support of  $\meas_{\alpha,\epsilon}$ has the same cardinality as as that of $\mestar$ and can be made arbitrarily close to $\Supp(\mestar)$. To obtain the required error bound, we exploit the implicit function theorem.

 


Define a function
$$
F:\RR_+^{\sum_s \abs{I_s}} \times \Tspace^k \times \RR^{T \times v}\times  \RR_+ \to \RR^{\sum_{s=1}^k \abs{I_s} + kd}
$$
by $F(C,\btheta,W,\alpha) = \begin{bmatrix}
\pa{g_i(C,\btheta,W,\alpha)}_{i=1}^k\\
\pa{h_i(C,\btheta,W,\alpha)}_{i=1}^k
\end{bmatrix}$
where writing $x\eqdef (C,\btheta,W,\alpha)$,
$$
g_s(x) = \proj_{I_s}
\pa{ \phi(\theta_s)^\top[D_\btheta \bar C^\top -D_{\btheta^*} (C^*)^\top - w ] }+ \alpha \pa{ \lambda_1 +  \lambda_2 \frac{C_s^\top}{\norm{C_s}}}
$$
and
$$
h_s(x) = J_{\phi}(\theta_s)^\top \pa{D_\btheta \bar C^\top - D_{\btheta^*} (C^*)^\top - W} \frac{C_s}{\norm{C_s}_2}.
$$
Here, $\bar C \in \RR^{ v\times k}$ is the matrix with $s^{th}$ column satisfying  $(\bar C_s)_{I_s} = C_s$ and $(\bar C_s)_{I_s^c} = 0$.
Clearly, if $(C,\btheta)$ correspond to a solution with data $y= D_{\btheta^*} (C^*)^\top + W$, then $F(C,\btheta,W,\alpha) = 0$. Note also that $F(C^*, \btheta^*, 0,0) = 0$.



Writing $x = (C,\btheta)$, $N= \sum_{s}\abs{I_s}$, $$\partial_x F(C^*,\btheta^*,0,0) = \Gamma_{\btheta^*,C^*}^\top \Gamma_{\btheta^*,C^*} \begin{pmatrix}
\Id_{N} & \mathbf{0}_{N \times kd}\\
\mathbf{0}_{kd\times N } &\diag\pa{\norm{C_s}_2}_{s=1}^k \otimes \Id_{d}
\end{pmatrix}
$$
By assumption, $\partial_x F$ is invertible. By the implicit function theorem, there exists neighbourhoods $\Xx \subset \RR_+^{kv} \times \Tspace^k$ of $(C^*, \btheta^*)$ and $\Yy \subset \RR^{Lv}\times \RR_+$ of $(0,0)$ and a unique  continuously differentiable function $g:\Yy \to \Xx$ such that $F(g(y), y) = 0$ for all $y = (W,\alpha)\in V$. Moreover, since $g$ is continuously differentiable, $\norm{g(y) - g(0)} \leq C \norm{y}$. In particular, writing $(C,\btheta) = g(y)$,
$$
\norm{C - C^*}_F+ \norm{\btheta - \btheta^*} \leq C (\alpha + \norm{W}_F) .
$$
Finally,  since we have already established support stability in Proposition \ref{prop:stability}, by uniqueness, $g(y)$ coincides with solutions of \eqref{eq:spglasso}.


\end{proof}


\section{Derivation of Algorithm \ref{alg:FW}}

%%%%%%%%%%%%%%%%%%%%%
We follow the presentation of \cite{denoyelle2019sliding} where the sliding Frank-Wolfe was presented for scalar-valued measures.
The Frank-Wolfe algorithm seeks to solve minimisation problems of the form 
$$
\min_{m\in \Kk} F(m)
$$
where $f:\Xx\to \RR$ is a continuously differentiable function defined on some Banach space $\Xx$, and $\Kk \subseteq \Xx$ is a bounded convex  set. To  derive our algorithm, we follow \cite{denoyelle2019sliding} by rewriting \eqref{eq:spglasso} as the minimisation of a differentiable function over a bounded convex set. Note that  the optimal measure satisfies
$$
\frac12 \norm{\Phi \meas - X}_F^2 +  \alpha \norm{\meas}_\beta  \leq \norm{X}_F^2/2
$$
Recalling the definition of $\norm{\cdot}_\beta$, we can write $ \alpha \norm{\meas}_\beta  = \lambda_1 \abs{\meas}_1+ \lambda_2 \abs{\meas}_2$ where $\lambda_1 = \alpha (1-\beta)$ and $\lambda_2 = \alpha \beta \sqrt{v}$.
So in particular, $\abs{\meas}_{1} \leq \norm{X}_F^2/\pa{2\lambda_1}$. We can therefore equivalently write this as
\begin{align*}
\min_{\meas\in\Mm_+(\Tspace;\RR^p), t_1,t_2\in\RR} F(t_1,t_2,\meas) \eqdef \lambda_1 t_1 + \lambda_2 t_2 + \frac12 \norm{\Phi\meas - y}^2
\\
\qquad \text{subject to } (t_1,t_2,\meas)\in \Kk
\end{align*}
where $\Kk\eqdef \enscond{(t_1,t_2,\meas)}{\abs{\meas}_1 \leq t_1,  \abs{\meas}_{2}\le t_2,  t_2 \leq t_1 \leq \frac{\norm{X}_F^2}{2\lambda_1}}$.
The differential of $F$ is a bounded linear operator on $\RR\times \RR \times \Mm_+(\Tspace;\RR^p)$. Writing $s \eqdef (t_1,t_2,\meas)$ and $s' \eqdef (t_1',t_2',\meas')$, we have  
$$
[\mathrm{d}F(s)]s' = \lambda_1 t_1' + \lambda_2 t_2' + \int [\Phi^*( \Phi \meas - y)] (\theta) \mathrm{d}\meas'(\theta)
$$
The Frank-Wolfe algorithm is an iterative algorithm consisting of the following two steps: Denoting the $k$th iterate by $x^k$, do
\begin{enumerate}
\item $
s^{k} \in \argmin_{s\in\Kk} \mathrm{d}F(x^k)(s)
$
\item $x^{k+1} = (1-\gamma_k) s^{k} +\gamma_k x_k$
\end{enumerate}
For the first step, we can restrict the minimisation to the the extremal points of the convex set $\Kk$, which are of the form $(\norm{M}_1, \norm{M}_2, M \delta_\theta)$ where $\theta\in \Tspace$ and $M\in \RR_+^v$. Therefore, writing $x^k = (t_1,t_2,\meas^k)$, we are led to solve
\begin{equation}\label{eq:tosolve}
(\theta,M) \in \argmin_{\theta\in\Tspace, M\in \RR^p_+}   \lambda_1 \norm{M}_1 + \lambda_2 \norm{M}_2 - \dotp{M}{\eta^k(\theta) }, 
\end{equation}
where $ \eta^k\eqdef -\Phi^*( \Phi \meas^k - y)$.
Let the optimal points be $M = (m_j)_{j=1}^v$ and $\theta$, then the optimality condition reads
$$
-\eta^k(\theta)_j + \lambda_2 \frac{m_j}{\norm{M}_2} + \lambda_1 = 0, \qquad \text{ if } m_j >0
$$
$$
\eta^k(\theta)_j \in [0, \lambda_1], \qquad \text{ if } m_j =0
$$
i.e. we have 
$$
  \frac{M}{\norm{M}_2} = \frac{1}{\lambda_2} \pa{  \eta^k(\theta) - \lambda_1}_+
$$
Plugging this back into \eqref{eq:tosolve} and simplifying, we are left with
\begin{align}
\theta \in  \argmax_{\theta\in\Tspace} 
     \sum_{i=1}^p \pa{  \eta^k(\theta)_i - \lambda_1}_+^2
\end{align}
The second step of the algorithm can be replaced by any procedure which improves the objective value, which leads to the optimization problems in lines 8 and 9 of Algorithm \ref{alg:FW}.
